Metropolitan Segment Traffic Speeds from Massive Floating Car Data in 10 Cities

Traffic analysis is crucial for urban operations and planning, while the availability of dense urban traffic data beyond loop detectors is still scarce. We present a large-scale floating vehicle dataset of per-street segment traffic information, Metropolitan Segment Traffic Speeds from Massive Floating Car Data in 10 Cities (MeTS-10), available for 10 global cities with a 15-minute resolution for collection periods ranging between 108 and 361 days in 2019-2021 and covering more than 1500 square kilometers per metropolitan area. MeTS-10 features traffic speed information at all street levels from main arterials to local streets for Antwerp, Bangkok, Barcelona, Berlin, Chicago, Istanbul, London, Madrid, Melbourne and Moscow. The dataset leverages the industrial-scale floating vehicle Traffic4cast data with speeds and vehicle counts provided in a privacy-preserving spatio-temporal aggregation. We detail the efficient matching approach mapping the data to the OpenStreetMap road graph. We evaluate the dataset by comparing it with publicly available stationary vehicle detector data (for Berlin, London, and Madrid) and the Uber traffic speed dataset (for Barcelona, Berlin, and London). The comparison highlights the differences across datasets in spatio-temporal coverage and variations in the reported traffic caused by the binning method. MeTS-10 enables novel, city-wide analysis of mobility and traffic patterns for ten major world cities, overcoming current limitations of spatially sparse vehicle detector data. The large spatial and temporal coverage offers an opportunity for joining the MeTS-10 with other datasets, such as traffic surveys in traffic planning studies or vehicle detector data in traffic control settings.

==> figures/speed_stats/speed_stats.tex <==
% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2020', 'output_folder': 'figures/speed_stats', 'city': ['berlin'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020
\clearpage\subsection{Key Figures Berlin (2020)}
\subsubsection{Road graph map Berlin (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_berlin_2020.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_berlin_2020.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Berlin (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_berlin_2020.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_berlin_2020.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Berlin (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_berlin_2020_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_berlin_2020_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Berlin (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_berlin_2020_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_berlin_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_berlin_2020_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_berlin_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_berlin_2020_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_berlin_2020_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020 / berlin
 num\_edges                &  &  &  &  &  &  88'882 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  288 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  457 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  82 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  77 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2739 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  159 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  10295 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  283 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  8455 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  61 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  1765 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  64221 &                                                \\
 num\_nodes                &  &  &  &  &  &  34308 &                                                 \\
 num\_edges\_per\_cell                & 1.0 & 0.2 & 1.0 & 1.0 & 8.0 &  405'500 &                                                 \\
 num\_intersecting\_cells                & 4.7 & 4.3 & 4.0 & 0.0 & 162.0 &  88'882 &                                                 \\
 node\_degree                & 2.9 & 0.9 & 3.0 & 1.0 & 6.0 &  34'308 &                                                 \\
 length\_meters                & 158.0 & 202.0 & 119.3 & 0.6 & 8'035.8 &  88'882 & 1.4e+07                                                \\
 \hspace{10pt}  motorway               & 1'053.6 & 1'216.8 & 585.6 & 31.0 & 6'833.6 &  288  & 3.0e+05                                                \\
 \hspace{10pt}  motorway\_link               & 240.2 & 222.8 & 209.6 & 12.1 & 1'744.2 &  457  & 1.1e+05                                                \\
 \hspace{10pt}  trunk               & 822.9 & 924.8 & 517.4 & 21.1 & 5'651.8 &  82  & 6.7e+04                                                \\
 \hspace{10pt}  trunk\_link               & 214.3 & 117.7 & 220.9 & 12.2 & 539.8 &  77  & 1.6e+04                                                \\
 \hspace{10pt}  primary               & 189.8 & 292.3 & 118.9 & 2.6 & 3'972.9 &  2'739  & 5.2e+05                                                \\
 \hspace{10pt}  primary\_link               & 85.7 & 170.6 & 19.9 & 7.0 & 1'303.9 &  159  & 1.4e+04                                                \\
 \hspace{10pt}  secondary               & 174.3 & 300.8 & 111.5 & 1.3 & 6'323.5 &  10'295  & 1.8e+06                                                \\
 \hspace{10pt}  secondary\_link               & 26.5 & 33.6 & 14.7 & 6.8 & 237.6 &  283  & 7.5e+03                                                \\
 \hspace{10pt}  tertiary               & 153.1 & 211.3 & 112.7 & 0.6 & 8'035.8 &  8'455  & 1.3e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 23.3 & 34.8 & 12.9 & 7.2 & 263.4 &  61  & 1.4e+03                                                \\
 \hspace{10pt}  unclassified               & 310.3 & 440.0 & 171.5 & 3.2 & 3'997.2 &  1'765  & 5.5e+05                                                \\
 \hspace{10pt}  residential               & 145.9 & 117.4 & 120.2 & 0.6 & 2'723.0 &  64'221  & 9.4e+06                                                \\
 speed\_kph                & 35.7 & 10.1 & 30.0 & 5.0 & 120.0 &  88'882 &                                                 \\
 \hspace{10pt}  motorway               & 85.4 & 17.3 & 80.0 & 40.0 & 120.0 &  288  &                                                 \\
 \hspace{10pt}  motorway\_link               & 61.2 & 14.0 & 60.0 & 30.0 & 120.0 &  457  &                                                 \\
 \hspace{10pt}  trunk               & 84.6 & 33.8 & 100.0 & 10.0 & 120.0 &  82  &                                                 \\
 \hspace{10pt}  trunk\_link               & 52.6 & 8.5 & 52.5 & 30.0 & 80.0 &  77  &                                                 \\
 \hspace{10pt}  primary               & 49.4 & 8.2 & 50.0 & 30.0 & 120.0 &  2'739  &                                                 \\
 \hspace{10pt}  primary\_link               & 49.5 & 9.0 & 50.0 & 30.0 & 100.0 &  159  &                                                 \\
 \hspace{10pt}  secondary               & 48.7 & 6.5 & 50.0 & 10.0 & 100.0 &  10'295  &                                                 \\
 \hspace{10pt}  secondary\_link               & 48.3 & 5.5 & 50.0 & 30.0 & 80.0 &  283  &                                                 \\
 \hspace{10pt}  tertiary               & 46.4 & 8.5 & 50.0 & 10.0 & 100.0 &  8'455  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 46.4 & 8.3 & 50.0 & 10.0 & 60.0 &  61  &                                                 \\
 \hspace{10pt}  unclassified               & 42.6 & 10.0 & 43.1 & 10.0 & 100.0 &  1'765  &                                                 \\
 \hspace{10pt}  residential               & 30.8 & 4.4 & 30.0 & 5.0 & 100.0 &  64'221  &                                                 \\
 free\_flow\_kph                & 37.5 & 14.1 & 35.3 & 0.0 & 120.0 &  85'244 &                                                 \\
 \hspace{10pt}  motorway               & 92.0 & 15.7 & 87.9 & 65.9 & 119.5 &  288  &                                                 \\
 \hspace{10pt}  motorway\_link               & 78.1 & 20.0 & 80.3 & 24.9 & 120.0 &  457  &                                                 \\
 \hspace{10pt}  trunk               & 87.7 & 26.3 & 96.7 & 27.9 & 118.4 &  82  &                                                 \\
 \hspace{10pt}  trunk\_link               & 83.8 & 26.4 & 82.2 & 17.2 & 118.0 &  77  &                                                 \\
 \hspace{10pt}  primary               & 48.7 & 12.0 & 48.5 & 17.4 & 110.7 &  2'737  &                                                 \\
 \hspace{10pt}  primary\_link               & 45.9 & 19.4 & 42.8 & 12.2 & 104.5 &  159  &                                                 \\
 \hspace{10pt}  secondary               & 46.9 & 11.3 & 47.5 & 10.4 & 118.6 &  10'289  &                                                 \\
 \hspace{10pt}  secondary\_link               & 34.8 & 17.0 & 33.3 & 8.0 & 88.6 &  283  &                                                 \\
 \hspace{10pt}  tertiary               & 44.3 & 10.6 & 43.8 & 0.0 & 116.9 &  8'453  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 32.7 & 14.7 & 35.3 & 11.3 & 60.2 &  59  &                                                 \\
 \hspace{10pt}  unclassified               & 44.1 & 17.0 & 42.8 & 0.0 & 119.3 &  1'698  &                                                 \\
 \hspace{10pt}  residential               & 33.6 & 11.9 & 32.0 & 0.0 & 120.0 &  60'662  &                                                 \\
 speed\_kph-free\_flow\_kph                & -1.6 & 12.6 & -0.6 & -90.0 & 66.6 &  85'244 &                                                 \\
 \hspace{10pt}  motorway               & -6.7 & 16.6 & -6.6 & -43.5 & 53.0 &  288  &                                                 \\
 \hspace{10pt}  motorway\_link               & -16.8 & 21.0 & -19.5 & -77.6 & 66.6 &  457  &                                                 \\
 \hspace{10pt}  trunk               & -3.0 & 14.5 & 0.1 & -37.5 & 47.1 &  82  &                                                 \\
 \hspace{10pt}  trunk\_link               & -31.2 & 25.8 & -29.3 & -65.5 & 35.3 &  77  &                                                 \\
 \hspace{10pt}  primary               & 0.7 & 10.7 & 0.6 & -53.8 & 34.2 &  2'737  &                                                 \\
 \hspace{10pt}  primary\_link               & 3.5 & 19.3 & 5.6 & -57.0 & 57.8 &  159  &                                                 \\
 \hspace{10pt}  secondary               & 1.8 & 11.5 & 1.1 & -68.6 & 61.2 &  10'289  &                                                 \\
 \hspace{10pt}  secondary\_link               & 13.5 & 17.9 & 14.7 & -38.6 & 47.8 &  283  &                                                 \\
 \hspace{10pt}  tertiary               & 2.2 & 11.4 & 2.0 & -66.9 & 50.0 &  8'453  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 13.6 & 19.2 & 13.5 & -50.1 & 36.7 &  59  &                                                 \\
 \hspace{10pt}  unclassified               & -1.5 & 18.0 & -0.2 & -76.2 & 66.1 &  1'698  &                                                 \\
 \hspace{10pt}  residential               & -2.7 & 12.3 & -1.5 & -90.0 & 41.5 &  60'662  &                                                 \\
 movie volume 00:00--24:00               &  6.3e+07 & 1.2e+07  & 6.4e+07 & 3.3e+07 & 7.7e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  4.7e+05 & 1.8e+05  & 4.1e+05 & 2.7e+05 & 9.7e+05 &  20 &                                                \\
 movie volume 03:00--06:00               &  4.1e+05 & 1.6e+05  & 3.5e+05 & 2.2e+05 & 8.5e+05 &  20 &                                                \\
 movie volume 06:00--09:00               &  3.9e+05 & 1.6e+05  & 3.5e+05 & 1.9e+05 & 7.8e+05 &  20 &                                                \\
 movie volume 09:00--12:00               &  4.5e+05 & 1.8e+05  & 4.8e+05 & 2.0e+05 & 7.3e+05 &  20 &                                                \\
 movie volume 12:00--15:00               &  6.9e+05 & 3.7e+05  & 5.7e+05 & 2.7e+05 & 1.3e+06 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.1e+06 & 5.1e+05  & 7.7e+05 & 4.5e+05 & 1.9e+06 &  20 &                                                \\
 movie volume 18:00--21:00               &  1.5e+06 & 6.5e+05  & 1.4e+06 & 4.3e+05 & 2.4e+06 &  20 &                                                \\
 movie volume 21:00--24:00               &  2.0e+06 & 8.3e+05  & 2.1e+06 & 3.7e+05 & 3.1e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2020', 'output_folder': 'figures/speed_stats', 'city': ['istanbul'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020
\clearpage\subsection{Key Figures Istanbul (2020)}
\subsubsection{Road graph map Istanbul (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_istanbul_2020.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_istanbul_2020.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Istanbul (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_istanbul_2020.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_istanbul_2020.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Istanbul (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_istanbul_2020_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_istanbul_2020_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Istanbul (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_istanbul_2020_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_istanbul_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_istanbul_2020_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_istanbul_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_istanbul_2020_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_istanbul_2020_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020 / istanbul
 num\_edges                &  &  &  &  &  &  270'109 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  341 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  695 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  1153 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  1527 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  9242 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  2439 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  17042 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  1392 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  30078 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  630 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  5500 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  200070 &                                                \\
 num\_nodes                &  &  &  &  &  &  102754 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.6 & 1.0 & 1.0 & 16.0 &  734'722 &                                                 \\
 num\_intersecting\_cells                & 3.1 & 2.9 & 2.0 & 0.0 & 301.0 &  270'109 &                                                 \\
 node\_degree                & 3.0 & 0.8 & 3.0 & 1.0 & 7.0 &  102'754 &                                                 \\
 length\_meters                & 81.9 & 135.0 & 53.3 & 0.2 & 14'514.7 &  270'109 & 2.2e+07                                                \\
 \hspace{10pt}  motorway               & 1'062.8 & 1'686.5 & 651.0 & 25.8 & 14'514.7 &  341  & 3.6e+05                                                \\
 \hspace{10pt}  motorway\_link               & 360.0 & 312.1 & 276.6 & 5.3 & 2'154.8 &  695  & 2.5e+05                                                \\
 \hspace{10pt}  trunk               & 393.3 & 522.8 & 215.5 & 4.7 & 6'138.0 &  1'153  & 4.5e+05                                                \\
 \hspace{10pt}  trunk\_link               & 162.8 & 150.6 & 126.8 & 2.1 & 1'345.4 &  1'527  & 2.5e+05                                                \\
 \hspace{10pt}  primary               & 104.9 & 160.5 & 57.2 & 1.1 & 2'582.2 &  9'242  & 9.7e+05                                                \\
 \hspace{10pt}  primary\_link               & 65.4 & 78.4 & 37.4 & 0.7 & 817.5 &  2'439  & 1.6e+05                                                \\
 \hspace{10pt}  secondary               & 74.8 & 128.2 & 42.2 & 0.2 & 3'416.4 &  17'042  & 1.3e+06                                                \\
 \hspace{10pt}  secondary\_link               & 47.2 & 73.9 & 27.8 & 0.4 & 1'650.5 &  1'392  & 6.6e+04                                                \\
 \hspace{10pt}  tertiary               & 72.3 & 147.6 & 43.6 & 0.6 & 6'579.2 &  30'078  & 2.2e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 30.5 & 32.4 & 20.1 & 3.4 & 255.2 &  630  & 1.9e+04                                                \\
 \hspace{10pt}  unclassified               & 223.0 & 378.7 & 106.2 & 2.5 & 5'256.2 &  5'500  & 1.2e+06                                                \\
 \hspace{10pt}  residential               & 74.6 & 67.7 & 55.0 & 0.2 & 2'836.7 &  200'070  & 1.5e+07                                                \\
 speed\_kph                & 35.4 & 6.2 & 33.2 & 10.0 & 120.0 &  270'109 &                                                 \\
 \hspace{10pt}  motorway               & 107.0 & 10.4 & 107.3 & 46.6 & 120.0 &  341  &                                                 \\
 \hspace{10pt}  motorway\_link               & 47.2 & 7.9 & 46.6 & 30.0 & 120.0 &  695  &                                                 \\
 \hspace{10pt}  trunk               & 75.3 & 10.7 & 76.4 & 30.0 & 120.0 &  1'153  &                                                 \\
 \hspace{10pt}  trunk\_link               & 42.3 & 4.8 & 42.4 & 20.0 & 120.0 &  1'527  &                                                 \\
 \hspace{10pt}  primary               & 44.9 & 4.5 & 44.9 & 20.0 & 107.3 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & 32.4 & 2.8 & 32.4 & 20.0 & 90.0 &  2'439  &                                                 \\
 \hspace{10pt}  secondary               & 38.1 & 2.9 & 38.1 & 20.0 & 80.0 &  17'042  &                                                 \\
 \hspace{10pt}  secondary\_link               & 30.4 & 1.7 & 30.6 & 20.0 & 50.0 &  1'392  &                                                 \\
 \hspace{10pt}  tertiary               & 45.1 & 2.1 & 45.2 & 20.0 & 90.0 &  30'078  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 31.8 & 1.9 & 31.6 & 20.0 & 50.0 &  630  &                                                 \\
 \hspace{10pt}  unclassified               & 22.6 & 2.1 & 22.3 & 20.0 & 45.2 &  5'500  &                                                 \\
 \hspace{10pt}  residential               & 33.2 & 1.1 & 33.2 & 10.0 & 80.0 &  200'070  &                                                 \\
 free\_flow\_kph                & 24.8 & 12.6 & 21.0 & 0.0 & 108.7 &  268'450 &                                                 \\
 \hspace{10pt}  motorway               & 81.4 & 14.1 & 83.5 & 19.3 & 107.5 &  341  &                                                 \\
 \hspace{10pt}  motorway\_link               & 69.7 & 16.7 & 72.3 & 12.7 & 101.4 &  694  &                                                 \\
 \hspace{10pt}  trunk               & 62.0 & 14.7 & 64.9 & 8.0 & 95.8 &  1'153  &                                                 \\
 \hspace{10pt}  trunk\_link               & 54.4 & 18.2 & 57.6 & 6.6 & 95.8 &  1'525  &                                                 \\
 \hspace{10pt}  primary               & 36.7 & 12.5 & 34.8 & 5.6 & 93.5 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & 33.9 & 14.1 & 32.0 & 0.0 & 93.5 &  2'439  &                                                 \\
 \hspace{10pt}  secondary               & 31.5 & 14.6 & 27.1 & 6.6 & 96.0 &  17'042  &                                                 \\
 \hspace{10pt}  secondary\_link               & 32.4 & 17.1 & 27.0 & 9.4 & 91.3 &  1'392  &                                                 \\
 \hspace{10pt}  tertiary               & 26.2 & 10.2 & 24.2 & 8.0 & 95.4 &  30'056  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 25.1 & 10.9 & 22.4 & 6.6 & 84.9 &  630  &                                                 \\
 \hspace{10pt}  unclassified               & 30.3 & 16.6 & 26.4 & 0.0 & 108.7 &  4'696  &                                                 \\
 \hspace{10pt}  residential               & 22.5 & 10.5 & 19.8 & 0.0 & 102.7 &  199'240  &                                                 \\
 speed\_kph-free\_flow\_kph                & 10.6 & 12.2 & 13.6 & -86.4 & 88.0 &  268'450 &                                                 \\
 \hspace{10pt}  motorway               & 25.6 & 15.5 & 23.6 & -14.8 & 88.0 &  341  &                                                 \\
 \hspace{10pt}  motorway\_link               & -22.5 & 17.3 & -24.9 & -59.4 & 36.7 &  694  &                                                 \\
 \hspace{10pt}  trunk               & 13.3 & 15.8 & 10.8 & -42.9 & 70.6 &  1'153  &                                                 \\
 \hspace{10pt}  trunk\_link               & -12.1 & 18.0 & -15.3 & -53.4 & 50.2 &  1'525  &                                                 \\
 \hspace{10pt}  primary               & 8.2 & 12.8 & 10.1 & -55.0 & 56.0 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & -1.5 & 14.2 & 0.4 & -61.1 & 48.6 &  2'439  &                                                 \\
 \hspace{10pt}  secondary               & 6.6 & 14.8 & 10.8 & -57.9 & 56.7 &  17'042  &                                                 \\
 \hspace{10pt}  secondary\_link               & -1.9 & 17.1 & 3.3 & -60.7 & 26.0 &  1'392  &                                                 \\
 \hspace{10pt}  tertiary               & 18.9 & 10.3 & 21.0 & -73.3 & 59.9 &  30'056  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 6.7 & 11.1 & 9.5 & -48.2 & 26.6 &  630  &                                                 \\
 \hspace{10pt}  unclassified               & -7.6 & 16.7 & -3.7 & -86.4 & 29.7 &  4'696  &                                                 \\
 \hspace{10pt}  residential               & 10.7 & 10.5 & 13.4 & -71.0 & 61.6 &  199'240  &                                                 \\
 movie volume 00:00--24:00               &  6.5e+07 & 1.7e+07  & 7.0e+07 & 2.9e+07 & 8.7e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  2.8e+05 & 8.2e+04  & 2.6e+05 & 1.9e+05 & 4.8e+05 &  20 &                                                \\
 movie volume 03:00--06:00               &  2.8e+05 & 8.5e+04  & 2.4e+05 & 1.7e+05 & 4.7e+05 &  20 &                                                \\
 movie volume 06:00--09:00               &  3.5e+05 & 8.8e+04  & 3.4e+05 & 2.4e+05 & 5.6e+05 &  20 &                                                \\
 movie volume 09:00--12:00               &  6.3e+05 & 1.6e+05  & 6.3e+05 & 3.2e+05 & 9.6e+05 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.5e+06 & 6.0e+05  & 1.8e+06 & 4.5e+05 & 2.3e+06 &  20 &                                                \\
 movie volume 15:00--18:00               &  2.7e+06 & 1.2e+06  & 3.2e+06 & 5.2e+05 & 4.1e+06 &  20 &                                                \\
 movie volume 18:00--21:00               &  3.3e+06 & 1.4e+06  & 3.8e+06 & 6.2e+05 & 5.1e+06 &  20 &                                                \\
 movie volume 21:00--24:00               &  3.0e+06 & 1.1e+06  & 3.3e+06 & 7.0e+05 & 4.5e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2020', 'output_folder': 'figures/speed_stats', 'city': ['moscow'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020
\clearpage\subsection{Key Figures Moscow (2020)}
\subsubsection{Road graph map Moscow (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_moscow_2020.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_moscow_2020.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Moscow (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_moscow_2020.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_moscow_2020.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Moscow (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_moscow_2020_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_moscow_2020_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Moscow (2020)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_moscow_2020_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_moscow_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_moscow_2020_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_moscow_2020_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_moscow_2020_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_moscow_2020_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2020 / moscow
 num\_edges                &  &  &  &  &  &  47'877 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  17 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  651 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  150 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2765 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  575 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  9404 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  1461 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  11176 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  808 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  6159 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  14711 &                                                \\
 num\_nodes                &  &  &  &  &  &  22627 &                                                 \\
 num\_edges\_per\_cell                & 1.0 & 0.2 & 1.0 & 1.0 & 8.0 &  293'771 &                                                 \\
 num\_intersecting\_cells                & 6.3 & 6.2 & 4.0 & 1.0 & 144.0 &  47'877 &                                                 \\
 node\_degree                & 2.9 & 0.8 & 3.0 & 1.0 & 7.0 &  22'627 &                                                 \\
 length\_meters                & 227.8 & 280.2 & 140.5 & 1.0 & 8'043.8 &  47'877 & 1.1e+07                                                \\
 \hspace{10pt}  motorway               & 2'098.2 & 2'177.2 & 741.0 & 151.3 & 7'024.4 &  17  & 3.6e+04                                                \\
 \hspace{10pt}  trunk               & 551.2 & 802.4 & 291.1 & 4.3 & 8'043.8 &  651  & 3.6e+05                                                \\
 \hspace{10pt}  trunk\_link               & 363.9 & 332.4 & 268.5 & 9.8 & 1'612.1 &  150  & 5.5e+04                                                \\
 \hspace{10pt}  primary               & 294.1 & 371.7 & 174.6 & 1.8 & 4'378.8 &  2'765  & 8.1e+05                                                \\
 \hspace{10pt}  primary\_link               & 238.1 & 242.6 & 164.0 & 3.8 & 1'689.3 &  575  & 1.4e+05                                                \\
 \hspace{10pt}  secondary               & 209.7 & 255.5 & 115.8 & 1.0 & 3'017.5 &  9'404  & 2.0e+06                                                \\
 \hspace{10pt}  secondary\_link               & 138.4 & 165.0 & 75.8 & 4.8 & 1'564.7 &  1'461  & 2.0e+05                                                \\
 \hspace{10pt}  tertiary               & 230.3 & 268.1 & 134.3 & 1.9 & 3'168.5 &  11'176  & 2.6e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 97.9 & 124.1 & 54.9 & 3.5 & 1'141.1 &  808  & 7.9e+04                                                \\
 \hspace{10pt}  unclassified               & 205.9 & 251.8 & 125.4 & 1.4 & 3'738.3 &  6'159  & 1.3e+06                                                \\
 \hspace{10pt}  residential               & 232.0 & 233.0 & 165.0 & 1.4 & 2'597.8 &  14'711  & 3.4e+06                                                \\
 speed\_kph                & 48.6 & 11.3 & 49.0 & 5.0 & 110.0 &  47'877 &                                                 \\
 \hspace{10pt}  motorway               & 73.1 & 15.9 & 73.2 & 40.0 & 110.0 &  17  &                                                 \\
 \hspace{10pt}  trunk               & 94.1 & 12.0 & 100.0 & 40.0 & 110.0 &  651  &                                                 \\
 \hspace{10pt}  trunk\_link               & 54.1 & 5.6 & 54.5 & 30.0 & 90.0 &  150  &                                                 \\
 \hspace{10pt}  primary               & 73.8 & 6.5 & 74.1 & 40.0 & 90.0 &  2'765  &                                                 \\
 \hspace{10pt}  primary\_link               & 45.2 & 4.7 & 45.1 & 20.0 & 60.0 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 53.5 & 5.5 & 53.5 & 20.0 & 90.0 &  9'404  &                                                 \\
 \hspace{10pt}  secondary\_link               & 50.6 & 3.8 & 50.4 & 20.0 & 90.0 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 49.6 & 5.3 & 49.0 & 5.0 & 90.0 &  11'176  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 52.6 & 3.2 & 52.4 & 30.0 & 90.0 &  808  &                                                 \\
 \hspace{10pt}  unclassified               & 36.7 & 5.2 & 36.6 & 5.0 & 90.0 &  6'159  &                                                 \\
 \hspace{10pt}  residential               & 42.5 & 4.5 & 42.6 & 5.0 & 90.0 &  14'711  &                                                 \\
 free\_flow\_kph                & 34.1 & 15.5 & 30.7 & 0.0 & 120.0 &  47'356 &                                                 \\
 \hspace{10pt}  motorway               & 91.1 & 10.9 & 90.4 & 75.1 & 108.7 &  17  &                                                 \\
 \hspace{10pt}  trunk               & 70.5 & 11.0 & 71.7 & 32.0 & 99.8 &  651  &                                                 \\
 \hspace{10pt}  trunk\_link               & 60.5 & 11.2 & 59.9 & 31.5 & 100.7 &  150  &                                                 \\
 \hspace{10pt}  primary               & 49.8 & 12.5 & 50.4 & 2.8 & 82.4 &  2'765  &                                                 \\
 \hspace{10pt}  primary\_link               & 51.0 & 13.0 & 51.9 & 8.0 & 79.4 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 40.0 & 12.5 & 38.6 & 1.3 & 120.0 &  9'403  &                                                 \\
 \hspace{10pt}  secondary\_link               & 45.0 & 15.0 & 45.0 & 3.8 & 87.5 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 34.7 & 11.9 & 32.7 & 0.0 & 120.0 &  11'172  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 42.6 & 17.6 & 41.5 & 2.0 & 102.7 &  808  &                                                 \\
 \hspace{10pt}  unclassified               & 28.3 & 13.6 & 25.4 & 0.0 & 91.9 &  6'087  &                                                 \\
 \hspace{10pt}  residential               & 25.1 & 12.2 & 22.4 & 0.0 & 111.3 &  14'267  &                                                 \\
 speed\_kph-free\_flow\_kph                & 14.5 & 14.1 & 16.7 & -71.0 & 87.2 &  47'356 &                                                 \\
 \hspace{10pt}  motorway               & -17.9 & 22.7 & -12.4 & -66.2 & 16.2 &  17  &                                                 \\
 \hspace{10pt}  trunk               & 23.6 & 12.9 & 25.2 & -44.4 & 61.9 &  651  &                                                 \\
 \hspace{10pt}  trunk\_link               & -6.4 & 12.2 & -5.8 & -46.2 & 24.0 &  150  &                                                 \\
 \hspace{10pt}  primary               & 23.9 & 12.1 & 22.8 & -22.0 & 87.2 &  2'765  &                                                 \\
 \hspace{10pt}  primary\_link               & -5.8 & 13.7 & -6.8 & -39.2 & 35.4 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 13.5 & 13.4 & 14.9 & -66.5 & 75.6 &  9'403  &                                                 \\
 \hspace{10pt}  secondary\_link               & 5.6 & 15.2 & 5.9 & -50.3 & 46.6 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 15.0 & 12.6 & 17.0 & -71.0 & 55.4 &  11'172  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 10.0 & 17.7 & 10.7 & -50.3 & 58.0 &  808  &                                                 \\
 \hspace{10pt}  unclassified               & 8.4 & 13.9 & 10.7 & -58.3 & 50.1 &  6'087  &                                                 \\
 \hspace{10pt}  residential               & 17.5 & 12.9 & 20.5 & -68.7 & 72.8 &  14'267  &                                                 \\
 movie volume 00:00--24:00               &  7.1e+07 & 6.8e+06  & 7.1e+07 & 5.8e+07 & 8.4e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  1.3e+06 & 2.5e+05  & 1.2e+06 & 1.0e+06 & 1.9e+06 &  20 &                                                \\
 movie volume 03:00--06:00               &  1.2e+06 & 2.1e+05  & 1.1e+06 & 9.6e+05 & 1.7e+06 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.2e+06 & 1.7e+05  & 1.2e+06 & 1.0e+06 & 1.6e+06 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.3e+06 & 1.6e+05  & 1.3e+06 & 1.0e+06 & 1.6e+06 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.5e+06 & 1.8e+05  & 1.5e+06 & 1.1e+06 & 1.8e+06 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.7e+06 & 2.2e+05  & 1.7e+06 & 1.2e+06 & 2.0e+06 &  20 &                                                \\
 movie volume 18:00--21:00               &  1.8e+06 & 2.8e+05  & 1.9e+06 & 1.3e+06 & 2.2e+06 &  20 &                                                \\
 movie volume 21:00--24:00               &  2.0e+06 & 3.1e+05  & 2.0e+06 & 1.4e+06 & 2.5e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['antwerp'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Antwerp (2021)}
\subsubsection{Road graph map Antwerp (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_antwerp_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_antwerp_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Antwerp (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_antwerp_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_antwerp_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Antwerp (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_antwerp_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_antwerp_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Antwerp (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_antwerp_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_antwerp_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_antwerp_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_antwerp_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_antwerp_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_antwerp_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / antwerp
 num\_edges                &  &  &  &  &  &  81'667 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  232 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  483 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  274 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  67 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2798 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  152 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  3348 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  69 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  10929 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  42 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  11700 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  51573 &                                                \\
 num\_nodes                &  &  &  &  &  &  34722 &                                                 \\
 num\_edges\_per\_cell                & 1.0 & 0.2 & 1.0 & 1.0 & 10.0 &  385'170 &                                                 \\
 num\_intersecting\_cells                & 4.9 & 5.1 & 4.0 & 1.0 & 184.0 &  81'667 &                                                 \\
 node\_degree                & 2.7 & 0.9 & 3.0 & 1.0 & 6.0 &  34'722 &                                                 \\
 length\_meters                & 169.4 & 240.4 & 100.8 & 0.4 & 8'344.2 &  81'667 & 1.4e+07                                                \\
 \hspace{10pt}  motorway               & 1'496.8 & 1'426.3 & 954.9 & 17.0 & 7'793.1 &  232  & 3.5e+05                                                \\
 \hspace{10pt}  motorway\_link               & 313.5 & 330.0 & 218.0 & 4.3 & 2'417.4 &  483  & 1.5e+05                                                \\
 \hspace{10pt}  trunk               & 370.6 & 468.1 & 184.0 & 7.4 & 2'771.3 &  274  & 1.0e+05                                                \\
 \hspace{10pt}  trunk\_link               & 162.4 & 156.1 & 121.7 & 15.4 & 955.8 &  67  & 1.1e+04                                                \\
 \hspace{10pt}  primary               & 201.6 & 273.3 & 106.4 & 1.5 & 3'493.6 &  2'798  & 5.6e+05                                                \\
 \hspace{10pt}  primary\_link               & 49.6 & 66.0 & 24.4 & 2.8 & 373.7 &  152  & 7.5e+03                                                \\
 \hspace{10pt}  secondary               & 171.1 & 246.4 & 95.5 & 1.3 & 3'643.9 &  3'348  & 5.7e+05                                                \\
 \hspace{10pt}  secondary\_link               & 63.1 & 69.7 & 42.6 & 6.7 & 319.6 &  69  & 4.4e+03                                                \\
 \hspace{10pt}  tertiary               & 176.7 & 237.1 & 103.4 & 1.2 & 4'595.5 &  10'929  & 1.9e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 52.2 & 42.7 & 39.7 & 15.8 & 256.6 &  42  & 2.2e+03                                                \\
 \hspace{10pt}  unclassified               & 299.4 & 348.2 & 184.3 & 0.5 & 8'344.2 &  11'700  & 3.5e+06                                                \\
 \hspace{10pt}  residential               & 128.7 & 137.1 & 92.4 & 0.4 & 2'771.8 &  51'573  & 6.6e+06                                                \\
 speed\_kph                & 42.0 & 12.0 & 36.3 & 10.0 & 120.0 &  81'667 &                                                 \\
 \hspace{10pt}  motorway               & 109.2 & 15.9 & 120.0 & 50.0 & 120.0 &  232  &                                                 \\
 \hspace{10pt}  motorway\_link               & 82.6 & 16.6 & 81.4 & 30.0 & 120.0 &  483  &                                                 \\
 \hspace{10pt}  trunk               & 77.9 & 14.4 & 70.0 & 50.0 & 120.0 &  274  &                                                 \\
 \hspace{10pt}  trunk\_link               & 61.5 & 9.0 & 61.2 & 50.0 & 90.0 &  67  &                                                 \\
 \hspace{10pt}  primary               & 61.7 & 11.0 & 66.5 & 30.0 & 90.0 &  2'798  &                                                 \\
 \hspace{10pt}  primary\_link               & 55.5 & 5.7 & 55.5 & 30.0 & 70.0 &  152  &                                                 \\
 \hspace{10pt}  secondary               & 56.0 & 9.4 & 50.0 & 30.0 & 90.0 &  3'348  &                                                 \\
 \hspace{10pt}  secondary\_link               & 58.4 & 7.9 & 59.2 & 30.0 & 90.0 &  69  &                                                 \\
 \hspace{10pt}  tertiary               & 49.6 & 9.7 & 50.0 & 30.0 & 90.0 &  10'929  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 49.7 & 7.0 & 48.9 & 30.0 & 70.0 &  42  &                                                 \\
 \hspace{10pt}  unclassified               & 48.1 & 6.6 & 48.2 & 10.0 & 90.0 &  11'700  &                                                 \\
 \hspace{10pt}  residential               & 36.1 & 6.8 & 36.3 & 10.0 & 90.0 &  51'573  &                                                 \\
 free\_flow\_kph                & 38.9 & 18.0 & 35.8 & 0.0 & 120.0 &  77'109 &                                                 \\
 \hspace{10pt}  motorway               & 109.6 & 12.9 & 117.1 & 48.2 & 120.0 &  232  &                                                 \\
 \hspace{10pt}  motorway\_link               & 87.4 & 28.5 & 93.9 & 19.3 & 120.0 &  483  &                                                 \\
 \hspace{10pt}  trunk               & 66.5 & 22.9 & 65.2 & 17.9 & 120.0 &  272  &                                                 \\
 \hspace{10pt}  trunk\_link               & 74.1 & 25.1 & 74.6 & 26.8 & 120.0 &  67  &                                                 \\
 \hspace{10pt}  primary               & 52.2 & 16.3 & 50.5 & 2.8 & 120.0 &  2'798  &                                                 \\
 \hspace{10pt}  primary\_link               & 41.4 & 23.1 & 36.8 & 5.6 & 98.5 &  148  &                                                 \\
 \hspace{10pt}  secondary               & 49.4 & 16.8 & 46.6 & 4.7 & 119.1 &  3'344  &                                                 \\
 \hspace{10pt}  secondary\_link               & 53.8 & 31.4 & 41.8 & 13.6 & 118.6 &  68  &                                                 \\
 \hspace{10pt}  tertiary               & 46.0 & 15.5 & 43.8 & 0.0 & 120.0 &  10'915  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 43.9 & 18.6 & 41.2 & 20.7 & 97.9 &  42  &                                                 \\
 \hspace{10pt}  unclassified               & 44.1 & 21.7 & 41.9 & 0.0 & 120.0 &  10'392  &                                                 \\
 \hspace{10pt}  residential               & 33.6 & 13.9 & 32.0 & 0.0 & 120.0 &  48'348  &                                                 \\
 speed\_kph-free\_flow\_kph                & 3.3 & 15.8 & 3.9 & -90.0 & 66.6 &  77'109 &                                                 \\
 \hspace{10pt}  motorway               & -0.4 & 11.9 & 1.4 & -59.2 & 28.5 &  232  &                                                 \\
 \hspace{10pt}  motorway\_link               & -4.9 & 28.8 & -6.8 & -68.4 & 66.6 &  483  &                                                 \\
 \hspace{10pt}  trunk               & 11.5 & 19.8 & 7.2 & -48.6 & 65.5 &  272  &                                                 \\
 \hspace{10pt}  trunk\_link               & -12.6 & 24.8 & -10.8 & -70.0 & 34.4 &  67  &                                                 \\
 \hspace{10pt}  primary               & 9.5 & 14.5 & 7.9 & -47.2 & 60.3 &  2'798  &                                                 \\
 \hspace{10pt}  primary\_link               & 14.1 & 23.7 & 15.5 & -48.5 & 57.3 &  148  &                                                 \\
 \hspace{10pt}  secondary               & 6.7 & 16.1 & 7.2 & -88.6 & 65.3 &  3'344  &                                                 \\
 \hspace{10pt}  secondary\_link               & 4.6 & 30.2 & 17.6 & -59.2 & 45.6 &  68  &                                                 \\
 \hspace{10pt}  tertiary               & 3.6 & 14.2 & 3.9 & -70.0 & 59.6 &  10'915  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 5.9 & 20.2 & 7.7 & -49.0 & 39.4 &  42  &                                                 \\
 \hspace{10pt}  unclassified               & 4.0 & 21.6 & 6.1 & -90.0 & 60.1 &  10'392  &                                                 \\
 \hspace{10pt}  residential               & 2.5 & 14.1 & 3.2 & -90.0 & 51.2 &  48'348  &                                                 \\
 movie volume 00:00--24:00               &  3.6e+06 & 1.1e+06  & 3.2e+06 & 1.8e+06 & 5.2e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  4.2e+04 & 9.0e+03  & 4.5e+04 & 2.2e+04 & 5.7e+04 &  20 &                                                \\
 movie volume 03:00--06:00               &  3.4e+04 & 7.1e+03  & 3.4e+04 & 1.9e+04 & 4.6e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  2.8e+04 & 5.3e+03  & 2.7e+04 & 1.5e+04 & 3.7e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  2.5e+04 & 4.4e+03  & 2.5e+04 & 1.3e+04 & 3.1e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  2.4e+04 & 3.5e+03  & 2.5e+04 & 1.7e+04 & 2.9e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  2.5e+04 & 4.9e+03  & 2.6e+04 & 1.6e+04 & 3.4e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  3.3e+04 & 1.2e+04  & 2.8e+04 & 1.6e+04 & 5.0e+04 &  20 &                                                \\
 movie volume 21:00--24:00               &  6.1e+04 & 3.2e+04  & 4.0e+04 & 1.8e+04 & 1.1e+05 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['bangkok'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Bangkok (2021)}
\subsubsection{Road graph map Bangkok (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_bangkok_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_bangkok_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Bangkok (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_bangkok_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_bangkok_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Bangkok (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_bangkok_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_bangkok_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Bangkok (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_bangkok_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_bangkok_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_bangkok_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_bangkok_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_bangkok_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_bangkok_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / bangkok
 num\_edges                &  &  &  &  &  &  694'818 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  378 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  878 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  1579 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  682 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  7160 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  1974 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  15319 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  1510 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  25096 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  342 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  16290 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  623610 &                                                \\
 num\_nodes                &  &  &  &  &  &  317797 &                                                 \\
 num\_edges\_per\_cell                & 1.2 & 0.7 & 1.0 & 1.0 & 18.0 &  1'827'614 &                                                 \\
 num\_intersecting\_cells                & 3.1 & 2.5 & 2.0 & 0.0 & 225.0 &  694'818 &                                                 \\
 node\_degree                & 2.3 & 1.1 & 3.0 & 1.0 & 6.0 &  317'797 &                                                 \\
 length\_meters                & 84.6 & 118.3 & 49.6 & 0.0 & 12'311.6 &  694'818 & 5.9e+07                                                \\
 \hspace{10pt}  motorway               & 1'443.2 & 1'511.9 & 961.7 & 12.7 & 12'311.6 &  378  & 5.5e+05                                                \\
 \hspace{10pt}  motorway\_link               & 366.4 & 357.8 & 297.5 & 3.0 & 4'243.1 &  878  & 3.2e+05                                                \\
 \hspace{10pt}  trunk               & 299.6 & 439.6 & 115.9 & 1.7 & 3'589.9 &  1'579  & 4.7e+05                                                \\
 \hspace{10pt}  trunk\_link               & 138.9 & 189.5 & 76.1 & 7.3 & 1'463.7 &  682  & 9.5e+04                                                \\
 \hspace{10pt}  primary               & 159.8 & 263.3 & 78.3 & 0.3 & 5'461.4 &  7'160  & 1.1e+06                                                \\
 \hspace{10pt}  primary\_link               & 112.9 & 202.2 & 52.6 & 1.1 & 5'658.0 &  1'974  & 2.2e+05                                                \\
 \hspace{10pt}  secondary               & 107.7 & 148.3 & 59.3 & 0.2 & 2'543.0 &  15'319  & 1.6e+06                                                \\
 \hspace{10pt}  secondary\_link               & 111.4 & 178.4 & 45.2 & 4.1 & 2'079.3 &  1'510  & 1.7e+05                                                \\
 \hspace{10pt}  tertiary               & 87.9 & 125.2 & 49.5 & 0.0 & 2'328.6 &  25'096  & 2.2e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 57.2 & 121.8 & 14.8 & 4.6 & 821.5 &  342  & 2.0e+04                                                \\
 \hspace{10pt}  unclassified               & 124.7 & 175.4 & 63.6 & 0.4 & 2'013.2 &  16'290  & 2.0e+06                                                \\
 \hspace{10pt}  residential               & 80.0 & 95.0 & 49.0 & 0.1 & 4'957.8 &  623'610  & 5.0e+07                                                \\
 speed\_kph                & 31.8 & 7.5 & 29.7 & 10.0 & 120.0 &  694'818 &                                                 \\
 \hspace{10pt}  motorway               & 108.3 & 10.6 & 109.0 & 40.0 & 120.0 &  378  &                                                 \\
 \hspace{10pt}  motorway\_link               & 40.6 & 0.0 & 40.6 & 40.0 & 40.6 &  878  &                                                 \\
 \hspace{10pt}  trunk               & 54.9 & 1.4 & 54.9 & 54.9 & 109.0 &  1'579  &                                                 \\
 \hspace{10pt}  trunk\_link               & 54.9 & 0.0 & 54.9 & 54.9 & 54.9 &  682  &                                                 \\
 \hspace{10pt}  primary               & 62.8 & 2.3 & 62.9 & 30.0 & 80.0 &  7'160  &                                                 \\
 \hspace{10pt}  primary\_link               & 43.8 & 1.4 & 43.8 & 30.0 & 67.0 &  1'974  &                                                 \\
 \hspace{10pt}  secondary               & 67.0 & 2.1 & 67.0 & 30.0 & 90.0 &  15'319  &                                                 \\
 \hspace{10pt}  secondary\_link               & 54.9 & 0.8 & 54.9 & 43.8 & 67.0 &  1'510  &                                                 \\
 \hspace{10pt}  tertiary               & 36.4 & 1.9 & 36.4 & 30.0 & 80.0 &  25'096  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 54.9 & 0.0 & 54.9 & 54.9 & 54.9 &  342  &                                                 \\
 \hspace{10pt}  unclassified               & 49.7 & 1.6 & 49.7 & 30.0 & 80.0 &  16'290  &                                                 \\
 \hspace{10pt}  residential               & 29.7 & 0.6 & 29.7 & 10.0 & 100.0 &  623'610  &                                                 \\
 free\_flow\_kph                & 34.9 & 24.3 & 29.6 & 0.0 & 120.0 &  350'957 &                                                 \\
 \hspace{10pt}  motorway               & 83.3 & 17.3 & 81.5 & 24.5 & 120.0 &  378  &                                                 \\
 \hspace{10pt}  motorway\_link               & 74.4 & 21.3 & 77.4 & 13.6 & 120.0 &  877  &                                                 \\
 \hspace{10pt}  trunk               & 57.1 & 16.0 & 53.6 & 11.3 & 94.6 &  1'579  &                                                 \\
 \hspace{10pt}  trunk\_link               & 63.6 & 19.9 & 68.7 & 0.2 & 96.9 &  682  &                                                 \\
 \hspace{10pt}  primary               & 54.5 & 17.6 & 51.8 & 6.6 & 120.0 &  7'156  &                                                 \\
 \hspace{10pt}  primary\_link               & 58.5 & 22.3 & 60.2 & 4.7 & 120.0 &  1'965  &                                                 \\
 \hspace{10pt}  secondary               & 54.1 & 20.1 & 50.8 & 5.6 & 120.0 &  15'314  &                                                 \\
 \hspace{10pt}  secondary\_link               & 59.0 & 22.4 & 60.7 & 4.7 & 120.0 &  1'507  &                                                 \\
 \hspace{10pt}  tertiary               & 44.3 & 19.9 & 40.0 & 0.0 & 120.0 &  24'594  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 50.9 & 21.8 & 49.2 & 8.9 & 120.0 &  327  &                                                 \\
 \hspace{10pt}  unclassified               & 41.8 & 20.9 & 37.6 & 0.0 & 120.0 &  13'506  &                                                 \\
 \hspace{10pt}  residential               & 31.5 & 23.7 & 26.4 & 0.0 & 120.0 &  283'072  &                                                 \\
 speed\_kph-free\_flow\_kph                & -1.2 & 23.5 & 3.3 & -100.0 & 84.5 &  350'957 &                                                 \\
 \hspace{10pt}  motorway               & 25.0 & 20.7 & 28.1 & -56.8 & 84.5 &  378  &                                                 \\
 \hspace{10pt}  motorway\_link               & -33.8 & 21.3 & -36.8 & -79.4 & 27.0 &  877  &                                                 \\
 \hspace{10pt}  trunk               & -2.2 & 16.1 & 1.3 & -39.7 & 58.2 &  1'579  &                                                 \\
 \hspace{10pt}  trunk\_link               & -8.7 & 19.9 & -13.8 & -42.0 & 54.7 &  682  &                                                 \\
 \hspace{10pt}  primary               & 8.3 & 17.4 & 11.1 & -57.1 & 63.1 &  7'156  &                                                 \\
 \hspace{10pt}  primary\_link               & -14.7 & 22.3 & -16.4 & -76.2 & 39.1 &  1'965  &                                                 \\
 \hspace{10pt}  secondary               & 12.9 & 20.2 & 16.4 & -53.0 & 61.4 &  15'314  &                                                 \\
 \hspace{10pt}  secondary\_link               & -4.0 & 22.4 & -5.8 & -65.1 & 50.2 &  1'507  &                                                 \\
 \hspace{10pt}  tertiary               & -7.9 & 19.8 & -3.6 & -90.0 & 36.4 &  24'594  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 4.0 & 21.8 & 5.7 & -65.1 & 46.0 &  327  &                                                 \\
 \hspace{10pt}  unclassified               & 7.9 & 20.9 & 12.1 & -70.3 & 74.4 &  13'506  &                                                 \\
 \hspace{10pt}  residential               & -1.8 & 23.7 & 3.3 & -100.0 & 50.1 &  283'072  &                                                 \\
 movie volume 00:00--24:00               &  4.6e+06 & 1.8e+06  & 4.6e+06 & 1.7e+06 & 7.3e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  6.7e+04 & 2.6e+04  & 7.5e+04 & 2.7e+04 & 1.0e+05 &  20 &                                                \\
 movie volume 03:00--06:00               &  6.1e+04 & 2.3e+04  & 6.5e+04 & 2.7e+04 & 9.7e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  5.6e+04 & 2.2e+04  & 6.3e+04 & 2.3e+04 & 9.1e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  5.3e+04 & 2.2e+04  & 5.9e+04 & 1.9e+04 & 8.8e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  5.3e+04 & 2.3e+04  & 5.9e+04 & 1.8e+04 & 9.2e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  6.3e+04 & 2.5e+04  & 7.0e+04 & 2.3e+04 & 1.1e+05 &  20 &                                                \\
 movie volume 18:00--21:00               &  8.0e+04 & 3.2e+04  & 8.8e+04 & 2.8e+04 & 1.3e+05 &  20 &                                                \\
 movie volume 21:00--24:00               &  1.0e+05 & 3.8e+04  & 1.1e+05 & 3.4e+04 & 1.6e+05 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['barcelona'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Barcelona (2021)}
\subsubsection{Road graph map Barcelona (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_barcelona_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_barcelona_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Barcelona (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_barcelona_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_barcelona_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Barcelona (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_barcelona_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_barcelona_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Barcelona (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_barcelona_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_barcelona_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_barcelona_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_barcelona_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_barcelona_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_barcelona_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / barcelona
 num\_edges                &  &  &  &  &  &  118'813 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  442 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  700 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  613 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  860 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2126 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  690 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  5525 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  879 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  14875 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  1250 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  3840 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  87013 &                                                \\
 num\_nodes                &  &  &  &  &  &  58106 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.4 & 1.0 & 1.0 & 11.0 &  410'314 &                                                 \\
 num\_intersecting\_cells                & 3.7 & 4.6 & 3.0 & 0.0 & 286.0 &  118'813 &                                                 \\
 node\_degree                & 3.0 & 0.8 & 3.0 & 1.0 & 6.0 &  58'106 &                                                 \\
 length\_meters                & 118.5 & 215.0 & 74.0 & 0.1 & 13'629.4 &  118'813 & 1.4e+07                                                \\
 \hspace{10pt}  motorway               & 987.6 & 954.8 & 708.9 & 12.4 & 6'956.0 &  442  & 4.4e+05                                                \\
 \hspace{10pt}  motorway\_link               & 315.6 & 295.8 & 262.0 & 4.8 & 2'833.8 &  700  & 2.2e+05                                                \\
 \hspace{10pt}  trunk               & 456.4 & 428.8 & 355.4 & 5.0 & 3'003.2 &  613  & 2.8e+05                                                \\
 \hspace{10pt}  trunk\_link               & 199.6 & 163.0 & 165.8 & 2.9 & 1'219.4 &  860  & 1.7e+05                                                \\
 \hspace{10pt}  primary               & 122.2 & 227.6 & 63.1 & 0.9 & 3'285.7 &  2'126  & 2.6e+05                                                \\
 \hspace{10pt}  primary\_link               & 81.5 & 106.4 & 45.4 & 1.0 & 1'386.9 &  690  & 5.6e+04                                                \\
 \hspace{10pt}  secondary               & 122.6 & 268.5 & 52.9 & 0.6 & 6'191.2 &  5'525  & 6.8e+05                                                \\
 \hspace{10pt}  secondary\_link               & 54.9 & 80.4 & 29.9 & 1.4 & 1'030.9 &  879  & 4.8e+04                                                \\
 \hspace{10pt}  tertiary               & 122.3 & 361.2 & 55.2 & 0.8 & 13'629.4 &  14'875  & 1.8e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 46.2 & 60.3 & 27.8 & 1.5 & 651.1 &  1'250  & 5.8e+04                                                \\
 \hspace{10pt}  unclassified               & 238.8 & 458.7 & 101.7 & 0.1 & 10'442.1 &  3'840  & 9.2e+05                                                \\
 \hspace{10pt}  residential               & 105.0 & 112.4 & 76.6 & 0.1 & 3'436.9 &  87'013  & 9.1e+06                                                \\
 speed\_kph                & 37.2 & 9.4 & 33.9 & 2.0 & 120.0 &  118'813 &                                                 \\
 \hspace{10pt}  motorway               & 100.0 & 19.9 & 100.0 & 40.0 & 120.0 &  442  &                                                 \\
 \hspace{10pt}  motorway\_link               & 63.7 & 13.6 & 63.3 & 33.9 & 120.0 &  700  &                                                 \\
 \hspace{10pt}  trunk               & 81.5 & 15.5 & 80.0 & 40.0 & 100.0 &  613  &                                                 \\
 \hspace{10pt}  trunk\_link               & 58.5 & 10.9 & 58.6 & 20.0 & 100.0 &  860  &                                                 \\
 \hspace{10pt}  primary               & 48.0 & 9.6 & 50.0 & 20.0 & 90.0 &  2'126  &                                                 \\
 \hspace{10pt}  primary\_link               & 46.8 & 7.0 & 50.0 & 20.0 & 80.0 &  690  &                                                 \\
 \hspace{10pt}  secondary               & 49.5 & 10.7 & 50.0 & 20.0 & 90.0 &  5'525  &                                                 \\
 \hspace{10pt}  secondary\_link               & 46.2 & 6.5 & 46.7 & 30.0 & 90.0 &  879  &                                                 \\
 \hspace{10pt}  tertiary               & 43.3 & 8.1 & 44.2 & 3.0 & 90.0 &  14'875  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 38.7 & 6.9 & 38.5 & 2.0 & 70.0 &  1'250  &                                                 \\
 \hspace{10pt}  unclassified               & 40.9 & 5.1 & 41.0 & 10.0 & 80.0 &  3'840  &                                                 \\
 \hspace{10pt}  residential               & 33.7 & 3.7 & 33.9 & 5.0 & 70.0 &  87'013  &                                                 \\
 free\_flow\_kph                & 34.5 & 21.6 & 29.6 & 0.0 & 120.0 &  103'177 &                                                 \\
 \hspace{10pt}  motorway               & 105.3 & 12.3 & 104.0 & 64.5 & 120.0 &  442  &                                                 \\
 \hspace{10pt}  motorway\_link               & 94.3 & 22.7 & 99.8 & 10.8 & 120.0 &  699  &                                                 \\
 \hspace{10pt}  trunk               & 87.4 & 16.0 & 89.9 & 33.2 & 120.0 &  613  &                                                 \\
 \hspace{10pt}  trunk\_link               & 81.6 & 20.2 & 86.6 & 6.6 & 120.0 &  858  &                                                 \\
 \hspace{10pt}  primary               & 47.1 & 18.6 & 42.8 & 0.0 & 117.4 &  2'126  &                                                 \\
 \hspace{10pt}  primary\_link               & 52.9 & 21.9 & 49.9 & 9.9 & 120.0 &  686  &                                                 \\
 \hspace{10pt}  secondary               & 43.6 & 17.3 & 39.5 & 0.0 & 120.0 &  5'519  &                                                 \\
 \hspace{10pt}  secondary\_link               & 44.4 & 19.4 & 40.9 & 8.9 & 120.0 &  865  &                                                 \\
 \hspace{10pt}  tertiary               & 39.0 & 18.4 & 34.8 & 0.0 & 120.0 &  14'706  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 42.9 & 22.7 & 36.7 & 0.0 & 120.0 &  1'215  &                                                 \\
 \hspace{10pt}  unclassified               & 42.1 & 26.0 & 35.3 & 0.0 & 120.0 &  3'228  &                                                 \\
 \hspace{10pt}  residential               & 29.7 & 18.6 & 26.4 & 0.0 & 120.0 &  72'220  &                                                 \\
 speed\_kph-free\_flow\_kph                & 3.1 & 19.4 & 6.6 & -98.6 & 75.2 &  103'177 &                                                 \\
 \hspace{10pt}  motorway               & -5.3 & 15.7 & 0.0 & -54.0 & 25.4 &  442  &                                                 \\
 \hspace{10pt}  motorway\_link               & -30.6 & 22.6 & -35.1 & -86.1 & 52.5 &  699  &                                                 \\
 \hspace{10pt}  trunk               & -5.9 & 13.1 & -4.0 & -67.6 & 32.3 &  613  &                                                 \\
 \hspace{10pt}  trunk\_link               & -23.1 & 21.1 & -28.0 & -88.7 & 54.4 &  858  &                                                 \\
 \hspace{10pt}  primary               & 0.9 & 17.5 & 3.9 & -87.4 & 50.0 &  2'126  &                                                 \\
 \hspace{10pt}  primary\_link               & -6.0 & 22.3 & -0.9 & -72.6 & 40.1 &  686  &                                                 \\
 \hspace{10pt}  secondary               & 5.9 & 17.3 & 8.4 & -86.7 & 75.2 &  5'519  &                                                 \\
 \hspace{10pt}  secondary\_link               & 1.7 & 19.1 & 4.4 & -73.3 & 43.3 &  865  &                                                 \\
 \hspace{10pt}  tertiary               & 4.3 & 18.8 & 7.8 & -97.6 & 56.4 &  14'706  &                                                 \\
 \hspace{10pt}  tertiary\_link               & -4.1 & 23.0 & 1.8 & -81.5 & 50.0 &  1'215  &                                                 \\
 \hspace{10pt}  unclassified               & -1.0 & 26.5 & 5.7 & -98.6 & 53.6 &  3'228  &                                                 \\
 \hspace{10pt}  residential               & 3.9 & 18.7 & 7.1 & -98.6 & 50.0 &  72'220  &                                                 \\
 movie volume 00:00--24:00               &  1.9e+06 & 6.9e+05  & 2.0e+06 & 6.3e+05 & 3.2e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  2.3e+04 & 7.0e+03  & 2.2e+04 & 1.3e+04 & 3.3e+04 &  20 &                                                \\
 movie volume 03:00--06:00               &  1.9e+04 & 5.1e+03  & 1.8e+04 & 1.3e+04 & 2.9e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.8e+04 & 4.9e+03  & 1.6e+04 & 1.2e+04 & 2.8e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.7e+04 & 3.9e+03  & 1.6e+04 & 1.1e+04 & 2.5e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.7e+04 & 3.7e+03  & 1.5e+04 & 1.2e+04 & 2.5e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.9e+04 & 3.7e+03  & 1.9e+04 & 1.4e+04 & 2.8e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  2.3e+04 & 5.3e+03  & 2.3e+04 & 1.5e+04 & 3.6e+04 &  20 &                                                \\
 movie volume 21:00--24:00               &  2.5e+04 & 6.6e+03  & 2.6e+04 & 1.5e+04 & 4.3e+04 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['berlin'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Berlin (2021)}
\subsubsection{Road graph map Berlin (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_berlin_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_berlin_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Berlin (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_berlin_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_berlin_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Berlin (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_berlin_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_berlin_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Berlin (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_berlin_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_berlin_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_berlin_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_berlin_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_berlin_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_berlin_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / berlin
 num\_edges                &  &  &  &  &  &  88'882 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  279 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  469 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  75 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  77 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2754 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  150 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  10292 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  280 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  8486 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  61 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  1766 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  64193 &                                                \\
 num\_nodes                &  &  &  &  &  &  34308 &                                                 \\
 num\_edges\_per\_cell                & 1.0 & 0.2 & 1.0 & 1.0 & 8.0 &  405'500 &                                                 \\
 num\_intersecting\_cells                & 4.7 & 4.3 & 4.0 & 0.0 & 162.0 &  88'882 &                                                 \\
 node\_degree                & 2.9 & 0.9 & 3.0 & 1.0 & 6.0 &  34'308 &                                                 \\
 length\_meters                & 158.0 & 202.0 & 119.3 & 0.6 & 8'035.8 &  88'882 & 1.4e+07                                                \\
 \hspace{10pt}  motorway               & 1'058.1 & 1'232.4 & 585.3 & 31.0 & 6'833.6 &  279  & 3.0e+05                                                \\
 \hspace{10pt}  motorway\_link               & 256.9 & 257.1 & 216.8 & 12.1 & 1'744.2 &  469  & 1.2e+05                                                \\
 \hspace{10pt}  trunk               & 846.4 & 959.8 & 516.8 & 21.1 & 5'651.8 &  75  & 6.3e+04                                                \\
 \hspace{10pt}  trunk\_link               & 214.3 & 117.7 & 220.9 & 12.2 & 539.8 &  77  & 1.6e+04                                                \\
 \hspace{10pt}  primary               & 191.6 & 292.9 & 119.1 & 2.6 & 3'972.9 &  2'754  & 5.3e+05                                                \\
 \hspace{10pt}  primary\_link               & 52.6 & 73.4 & 18.0 & 7.0 & 329.6 &  150  & 7.9e+03                                                \\
 \hspace{10pt}  secondary               & 174.3 & 300.9 & 111.5 & 1.3 & 6'323.5 &  10'292  & 1.8e+06                                                \\
 \hspace{10pt}  secondary\_link               & 25.5 & 31.5 & 14.6 & 6.8 & 237.6 &  280  & 7.1e+03                                                \\
 \hspace{10pt}  tertiary               & 155.1 & 216.5 & 113.0 & 0.6 & 8'035.8 &  8'486  & 1.3e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 23.3 & 34.8 & 12.9 & 7.2 & 263.4 &  61  & 1.4e+03                                                \\
 \hspace{10pt}  unclassified               & 310.2 & 439.8 & 171.5 & 3.2 & 3'997.2 &  1'766  & 5.5e+05                                                \\
 \hspace{10pt}  residential               & 145.6 & 116.1 & 120.1 & 0.6 & 2'723.0 &  64'193  & 9.3e+06                                                \\
 speed\_kph                & 35.7 & 10.1 & 30.0 & 5.0 & 120.0 &  88'882 &                                                 \\
 \hspace{10pt}  motorway               & 85.4 & 17.1 & 80.0 & 60.0 & 120.0 &  279  &                                                 \\
 \hspace{10pt}  motorway\_link               & 61.7 & 14.7 & 60.0 & 30.0 & 120.0 &  469  &                                                 \\
 \hspace{10pt}  trunk               & 87.5 & 32.5 & 100.0 & 30.0 & 120.0 &  75  &                                                 \\
 \hspace{10pt}  trunk\_link               & 52.6 & 8.5 & 52.5 & 30.0 & 80.0 &  77  &                                                 \\
 \hspace{10pt}  primary               & 49.5 & 8.3 & 50.0 & 30.0 & 120.0 &  2'754  &                                                 \\
 \hspace{10pt}  primary\_link               & 48.9 & 7.8 & 50.0 & 30.0 & 70.0 &  150  &                                                 \\
 \hspace{10pt}  secondary               & 48.7 & 6.5 & 50.0 & 10.0 & 100.0 &  10'292  &                                                 \\
 \hspace{10pt}  secondary\_link               & 48.2 & 5.2 & 50.0 & 30.0 & 60.0 &  280  &                                                 \\
 \hspace{10pt}  tertiary               & 46.4 & 8.5 & 50.0 & 10.0 & 100.0 &  8'486  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 46.4 & 8.3 & 50.0 & 10.0 & 60.0 &  61  &                                                 \\
 \hspace{10pt}  unclassified               & 42.6 & 10.0 & 43.1 & 10.0 & 100.0 &  1'766  &                                                 \\
 \hspace{10pt}  residential               & 30.8 & 4.4 & 30.0 & 5.0 & 100.0 &  64'193  &                                                 \\
 free\_flow\_kph                & 37.4 & 14.1 & 35.3 & 0.0 & 120.0 &  85'074 &                                                 \\
 \hspace{10pt}  motorway               & 92.2 & 15.7 & 87.8 & 65.1 & 120.0 &  279  &                                                 \\
 \hspace{10pt}  motorway\_link               & 78.4 & 20.0 & 80.6 & 24.7 & 120.0 &  469  &                                                 \\
 \hspace{10pt}  trunk               & 90.5 & 25.2 & 99.1 & 43.0 & 118.6 &  75  &                                                 \\
 \hspace{10pt}  trunk\_link               & 83.7 & 26.8 & 82.4 & 18.6 & 118.4 &  77  &                                                 \\
 \hspace{10pt}  primary               & 48.8 & 12.1 & 48.5 & 12.0 & 112.2 &  2'754  &                                                 \\
 \hspace{10pt}  primary\_link               & 44.8 & 18.5 & 41.9 & 13.2 & 102.9 &  150  &                                                 \\
 \hspace{10pt}  secondary               & 46.9 & 11.3 & 47.5 & 10.4 & 118.7 &  10'283  &                                                 \\
 \hspace{10pt}  secondary\_link               & 34.8 & 16.7 & 33.6 & 8.9 & 89.4 &  280  &                                                 \\
 \hspace{10pt}  tertiary               & 44.2 & 10.7 & 43.8 & 0.0 & 117.0 &  8'484  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 32.8 & 15.1 & 33.4 & 11.3 & 62.2 &  59  &                                                 \\
 \hspace{10pt}  unclassified               & 43.9 & 17.0 & 42.8 & 1.9 & 120.0 &  1'689  &                                                 \\
 \hspace{10pt}  residential               & 33.4 & 11.8 & 32.0 & 0.0 & 120.0 &  60'475  &                                                 \\
 speed\_kph-free\_flow\_kph                & -1.5 & 12.6 & -0.6 & -90.0 & 67.1 &  85'074 &                                                 \\
 \hspace{10pt}  motorway               & -6.9 & 16.6 & -6.6 & -49.2 & 52.5 &  279  &                                                 \\
 \hspace{10pt}  motorway\_link               & -16.7 & 20.9 & -19.2 & -77.0 & 67.1 &  469  &                                                 \\
 \hspace{10pt}  trunk               & -3.0 & 13.4 & 0.1 & -34.7 & 49.1 &  75  &                                                 \\
 \hspace{10pt}  trunk\_link               & -31.1 & 26.1 & -29.8 & -65.9 & 33.9 &  77  &                                                 \\
 \hspace{10pt}  primary               & 0.7 & 10.8 & 0.5 & -54.0 & 39.1 &  2'754  &                                                 \\
 \hspace{10pt}  primary\_link               & 4.1 & 19.6 & 7.2 & -58.3 & 56.8 &  150  &                                                 \\
 \hspace{10pt}  secondary               & 1.8 & 11.5 & 1.1 & -68.7 & 61.2 &  10'283  &                                                 \\
 \hspace{10pt}  secondary\_link               & 13.4 & 17.9 & 15.3 & -39.4 & 47.3 &  280  &                                                 \\
 \hspace{10pt}  tertiary               & 2.2 & 11.4 & 2.2 & -70.5 & 50.0 &  8'484  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 13.5 & 19.6 & 14.6 & -51.6 & 38.2 &  59  &                                                 \\
 \hspace{10pt}  unclassified               & -1.3 & 18.1 & 0.3 & -76.0 & 66.1 &  1'689  &                                                 \\
 \hspace{10pt}  residential               & -2.5 & 12.3 & -1.3 & -90.0 & 42.9 &  60'475  &                                                 \\
 movie volume 00:00--24:00               &  5.9e+07 & 1.2e+07  & 5.4e+07 & 3.4e+07 & 7.7e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  8.8e+05 & 2.9e+05  & 8.6e+05 & 3.9e+05 & 1.5e+06 &  20 &                                                \\
 movie volume 03:00--06:00               &  7.0e+05 & 2.6e+05  & 6.8e+05 & 2.9e+05 & 1.2e+06 &  20 &                                                \\
 movie volume 06:00--09:00               &  5.8e+05 & 2.1e+05  & 5.5e+05 & 2.4e+05 & 9.7e+05 &  20 &                                                \\
 movie volume 09:00--12:00               &  5.1e+05 & 2.1e+05  & 4.5e+05 & 2.1e+05 & 9.1e+05 &  20 &                                                \\
 movie volume 12:00--15:00               &  4.7e+05 & 1.9e+05  & 4.3e+05 & 2.2e+05 & 8.7e+05 &  20 &                                                \\
 movie volume 15:00--18:00               &  4.8e+05 & 1.5e+05  & 4.4e+05 & 2.4e+05 & 7.4e+05 &  20 &                                                \\
 movie volume 18:00--21:00               &  6.2e+05 & 1.1e+05  & 6.6e+05 & 4.4e+05 & 8.2e+05 &  20 &                                                \\
 movie volume 21:00--24:00               &  9.7e+05 & 3.3e+05  & 1.0e+06 & 4.4e+05 & 1.5e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['chicago'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Chicago (2021)}
\subsubsection{Road graph map Chicago (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_chicago_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_chicago_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Chicago (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_chicago_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_chicago_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Chicago (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_chicago_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_chicago_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Chicago (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_chicago_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_chicago_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_chicago_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_chicago_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_chicago_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_chicago_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / chicago
 num\_edges                &  &  &  &  &  &  187'570 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  822 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  1178 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  207 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  73 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  10439 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  387 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  22812 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  208 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  16603 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  71 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  1069 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  133701 &                                                \\
 num\_nodes                &  &  &  &  &  &  68430 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.3 & 1.0 & 1.0 & 11.0 &  966'289 &                                                 \\
 num\_intersecting\_cells                & 5.5 & 3.3 & 4.0 & 0.0 & 119.0 &  187'570 &                                                 \\
 node\_degree                & 3.2 & 0.9 & 3.0 & 1.0 & 7.0 &  68'430 &                                                 \\
 length\_meters                & 144.6 & 134.2 & 103.9 & 0.4 & 7'471.5 &  187'570 & 2.7e+07                                                \\
 \hspace{10pt}  motorway               & 778.1 & 872.2 & 559.2 & 17.5 & 7'471.5 &  822  & 6.4e+05                                                \\
 \hspace{10pt}  motorway\_link               & 329.9 & 265.3 & 301.3 & 2.7 & 2'611.5 &  1'178  & 3.9e+05                                                \\
 \hspace{10pt}  trunk               & 370.4 & 431.5 & 262.0 & 5.7 & 2'528.8 &  207  & 7.7e+04                                                \\
 \hspace{10pt}  trunk\_link               & 106.8 & 102.1 & 59.3 & 4.1 & 373.5 &  73  & 7.8e+03                                                \\
 \hspace{10pt}  primary               & 141.9 & 158.8 & 102.1 & 1.0 & 3'758.8 &  10'439  & 1.5e+06                                                \\
 \hspace{10pt}  primary\_link               & 70.4 & 72.8 & 52.5 & 9.5 & 614.3 &  387  & 2.7e+04                                                \\
 \hspace{10pt}  secondary               & 128.0 & 111.6 & 101.5 & 0.4 & 1'676.8 &  22'812  & 2.9e+06                                                \\
 \hspace{10pt}  secondary\_link               & 61.2 & 66.2 & 43.8 & 3.5 & 369.7 &  208  & 1.3e+04                                                \\
 \hspace{10pt}  tertiary               & 140.2 & 148.4 & 102.3 & 1.0 & 5'115.0 &  16'603  & 2.3e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 40.3 & 31.5 & 30.6 & 6.4 & 144.7 &  71  & 2.9e+03                                                \\
 \hspace{10pt}  unclassified               & 229.4 & 297.9 & 126.5 & 3.5 & 2'156.3 &  1'069  & 2.5e+05                                                \\
 \hspace{10pt}  residential               & 142.0 & 95.5 & 106.8 & 1.4 & 3'849.4 &  133'701  & 1.9e+07                                                \\
 speed\_kph                & 41.0 & 8.0 & 36.8 & 16.1 & 112.7 &  187'570 &                                                 \\
 \hspace{10pt}  motorway               & 87.7 & 6.9 & 88.5 & 56.3 & 112.7 &  822  &                                                 \\
 \hspace{10pt}  motorway\_link               & 83.7 & 3.0 & 83.8 & 24.1 & 112.7 &  1'178  &                                                 \\
 \hspace{10pt}  trunk               & 75.1 & 8.8 & 74.4 & 48.3 & 88.5 &  207  &                                                 \\
 \hspace{10pt}  trunk\_link               & 57.1 & 0.0 & 57.1 & 57.1 & 57.1 &  73  &                                                 \\
 \hspace{10pt}  primary               & 55.6 & 3.4 & 55.8 & 36.8 & 88.5 &  10'439  &                                                 \\
 \hspace{10pt}  primary\_link               & 57.1 & 0.0 & 57.1 & 57.1 & 57.1 &  387  &                                                 \\
 \hspace{10pt}  secondary               & 50.9 & 1.9 & 50.9 & 24.1 & 74.4 &  22'812  &                                                 \\
 \hspace{10pt}  secondary\_link               & 32.2 & 0.0 & 32.2 & 32.2 & 32.2 &  208  &                                                 \\
 \hspace{10pt}  tertiary               & 44.7 & 2.5 & 44.7 & 32.2 & 83.8 &  16'603  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 48.3 & 0.0 & 48.3 & 48.3 & 48.3 &  71  &                                                 \\
 \hspace{10pt}  unclassified               & 56.3 & 2.7 & 56.3 & 40.2 & 88.5 &  1'069  &                                                 \\
 \hspace{10pt}  residential               & 36.8 & 0.6 & 36.8 & 16.1 & 72.4 &  133'701  &                                                 \\
 free\_flow\_kph                & 45.1 & 19.0 & 42.8 & 0.0 & 120.0 &  162'191 &                                                 \\
 \hspace{10pt}  motorway               & 99.4 & 12.9 & 98.1 & 35.9 & 120.0 &  822  &                                                 \\
 \hspace{10pt}  motorway\_link               & 91.4 & 20.9 & 95.5 & 14.6 & 120.0 &  1'178  &                                                 \\
 \hspace{10pt}  trunk               & 68.8 & 17.9 & 70.6 & 20.4 & 99.8 &  207  &                                                 \\
 \hspace{10pt}  trunk\_link               & 67.4 & 17.8 & 76.7 & 20.4 & 91.8 &  73  &                                                 \\
 \hspace{10pt}  primary               & 55.2 & 13.6 & 54.1 & 6.6 & 118.1 &  10'427  &                                                 \\
 \hspace{10pt}  primary\_link               & 52.4 & 17.2 & 51.8 & 0.0 & 112.0 &  384  &                                                 \\
 \hspace{10pt}  secondary               & 49.6 & 14.6 & 46.6 & 0.0 & 120.0 &  22'787  &                                                 \\
 \hspace{10pt}  secondary\_link               & 51.7 & 21.0 & 48.5 & 0.0 & 113.9 &  208  &                                                 \\
 \hspace{10pt}  tertiary               & 48.9 & 16.7 & 45.6 & 0.0 & 120.0 &  16'538  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 48.4 & 20.2 & 46.6 & 14.6 & 113.6 &  69  &                                                 \\
 \hspace{10pt}  unclassified               & 47.6 & 24.9 & 46.5 & 2.4 & 120.0 &  988  &                                                 \\
 \hspace{10pt}  residential               & 41.5 & 18.5 & 39.2 & 0.0 & 120.0 &  108'510  &                                                 \\
 speed\_kph-free\_flow\_kph                & -3.4 & 17.7 & -0.9 & -85.5 & 69.2 &  162'191 &                                                 \\
 \hspace{10pt}  motorway               & -11.8 & 12.8 & -10.6 & -53.3 & 52.2 &  822  &                                                 \\
 \hspace{10pt}  motorway\_link               & -7.7 & 21.0 & -11.7 & -85.5 & 69.2 &  1'178  &                                                 \\
 \hspace{10pt}  trunk               & 6.3 & 14.9 & 3.7 & -25.4 & 54.0 &  207  &                                                 \\
 \hspace{10pt}  trunk\_link               & -10.3 & 17.8 & -19.6 & -34.7 & 36.7 &  73  &                                                 \\
 \hspace{10pt}  primary               & 0.4 & 13.3 & 1.2 & -62.3 & 49.7 &  10'427  &                                                 \\
 \hspace{10pt}  primary\_link               & 4.7 & 17.2 & 5.3 & -54.9 & 57.1 &  384  &                                                 \\
 \hspace{10pt}  secondary               & 1.2 & 14.6 & 4.1 & -69.9 & 50.9 &  22'787  &                                                 \\
 \hspace{10pt}  secondary\_link               & -19.5 & 21.0 & -16.3 & -81.7 & 32.2 &  208  &                                                 \\
 \hspace{10pt}  tertiary               & -4.2 & 16.7 & -1.2 & -76.4 & 44.7 &  16'538  &                                                 \\
 \hspace{10pt}  tertiary\_link               & -0.1 & 20.2 & 1.7 & -65.3 & 33.7 &  69  &                                                 \\
 \hspace{10pt}  unclassified               & 8.7 & 24.8 & 9.7 & -63.7 & 53.9 &  988  &                                                 \\
 \hspace{10pt}  residential               & -4.7 & 18.5 & -2.3 & -83.9 & 40.2 &  108'510  &                                                 \\
 movie volume 00:00--24:00               &  4.1e+06 & 2.0e+06  & 3.5e+06 & 7.1e+04 & 7.6e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  2.8e+04 & 1.8e+04  & 2.6e+04 & 0.0e+00 & 7.6e+04 &  20 &                                                \\
 movie volume 03:00--06:00               &  2.2e+04 & 1.4e+04  & 2.0e+04 & 0.0e+00 & 4.9e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.8e+04 & 1.1e+04  & 1.9e+04 & 0.0e+00 & 4.0e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.6e+04 & 8.6e+03  & 1.7e+04 & 0.0e+00 & 3.3e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.7e+04 & 8.5e+03  & 1.9e+04 & 0.0e+00 & 3.1e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  2.1e+04 & 1.1e+04  & 2.6e+04 & 0.0e+00 & 4.1e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  2.9e+04 & 1.6e+04  & 3.0e+04 & 0.0e+00 & 5.3e+04 &  20 &                                                \\
 movie volume 21:00--24:00               &  5.2e+04 & 3.2e+04  & 4.6e+04 & 0.0e+00 & 9.9e+04 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['istanbul'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Istanbul (2021)}
\subsubsection{Road graph map Istanbul (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_istanbul_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_istanbul_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Istanbul (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_istanbul_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_istanbul_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Istanbul (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_istanbul_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_istanbul_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Istanbul (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_istanbul_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_istanbul_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_istanbul_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_istanbul_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_istanbul_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_istanbul_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / istanbul
 num\_edges                &  &  &  &  &  &  270'109 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  338 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  699 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  1156 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  1529 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  9242 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  2430 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  17014 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  1403 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  30221 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  625 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  5422 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  200030 &                                                \\
 num\_nodes                &  &  &  &  &  &  102754 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.6 & 1.0 & 1.0 & 16.0 &  734'722 &                                                 \\
 num\_intersecting\_cells                & 3.1 & 2.9 & 2.0 & 0.0 & 301.0 &  270'109 &                                                 \\
 node\_degree                & 3.0 & 0.8 & 3.0 & 1.0 & 7.0 &  102'754 &                                                 \\
 length\_meters                & 81.9 & 135.0 & 53.3 & 0.2 & 14'514.7 &  270'109 & 2.2e+07                                                \\
 \hspace{10pt}  motorway               & 1'066.1 & 1'693.6 & 647.9 & 25.8 & 14'514.7 &  338  & 3.6e+05                                                \\
 \hspace{10pt}  motorway\_link               & 361.1 & 312.1 & 277.1 & 5.3 & 2'154.8 &  699  & 2.5e+05                                                \\
 \hspace{10pt}  trunk               & 394.2 & 522.6 & 216.3 & 4.7 & 6'138.0 &  1'156  & 4.6e+05                                                \\
 \hspace{10pt}  trunk\_link               & 162.4 & 148.9 & 126.8 & 2.1 & 1'345.4 &  1'529  & 2.5e+05                                                \\
 \hspace{10pt}  primary               & 104.8 & 160.3 & 57.2 & 1.1 & 2'582.2 &  9'242  & 9.7e+05                                                \\
 \hspace{10pt}  primary\_link               & 65.0 & 78.0 & 37.4 & 0.7 & 817.5 &  2'430  & 1.6e+05                                                \\
 \hspace{10pt}  secondary               & 74.6 & 128.1 & 42.2 & 0.2 & 3'416.4 &  17'014  & 1.3e+06                                                \\
 \hspace{10pt}  secondary\_link               & 48.6 & 75.7 & 28.1 & 0.4 & 1'650.5 &  1'403  & 6.8e+04                                                \\
 \hspace{10pt}  tertiary               & 73.5 & 153.4 & 43.8 & 0.6 & 6'579.2 &  30'221  & 2.2e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 30.4 & 32.4 & 20.1 & 3.4 & 251.3 &  625  & 1.9e+04                                                \\
 \hspace{10pt}  unclassified               & 217.9 & 370.2 & 104.7 & 2.5 & 5'256.2 &  5'422  & 1.2e+06                                                \\
 \hspace{10pt}  residential               & 74.6 & 67.7 & 55.0 & 0.2 & 2'438.5 &  200'030  & 1.5e+07                                                \\
 speed\_kph                & 35.4 & 6.2 & 33.2 & 10.0 & 120.0 &  270'109 &                                                 \\
 \hspace{10pt}  motorway               & 107.1 & 9.9 & 107.3 & 50.0 & 120.0 &  338  &                                                 \\
 \hspace{10pt}  motorway\_link               & 47.5 & 8.8 & 46.6 & 30.0 & 120.0 &  699  &                                                 \\
 \hspace{10pt}  trunk               & 75.3 & 10.8 & 76.4 & 30.0 & 120.0 &  1'156  &                                                 \\
 \hspace{10pt}  trunk\_link               & 42.3 & 4.8 & 42.4 & 20.0 & 120.0 &  1'529  &                                                 \\
 \hspace{10pt}  primary               & 44.9 & 4.5 & 44.9 & 20.0 & 90.0 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & 32.4 & 2.8 & 32.4 & 20.0 & 90.0 &  2'430  &                                                 \\
 \hspace{10pt}  secondary               & 38.1 & 2.9 & 38.1 & 20.0 & 80.0 &  17'014  &                                                 \\
 \hspace{10pt}  secondary\_link               & 30.5 & 1.8 & 30.6 & 20.0 & 50.0 &  1'403  &                                                 \\
 \hspace{10pt}  tertiary               & 45.1 & 2.2 & 45.2 & 20.0 & 90.0 &  30'221  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 31.6 & 1.4 & 31.6 & 20.0 & 50.0 &  625  &                                                 \\
 \hspace{10pt}  unclassified               & 22.4 & 1.2 & 22.3 & 20.0 & 33.2 &  5'422  &                                                 \\
 \hspace{10pt}  residential               & 33.2 & 1.1 & 33.2 & 10.0 & 80.0 &  200'030  &                                                 \\
 free\_flow\_kph                & 24.7 & 12.4 & 20.9 & 0.0 & 108.9 &  268'548 &                                                 \\
 \hspace{10pt}  motorway               & 81.4 & 14.2 & 83.9 & 16.0 & 108.9 &  338  &                                                 \\
 \hspace{10pt}  motorway\_link               & 69.4 & 16.7 & 71.7 & 13.2 & 101.2 &  698  &                                                 \\
 \hspace{10pt}  trunk               & 61.7 & 14.7 & 64.5 & 5.6 & 95.5 &  1'156  &                                                 \\
 \hspace{10pt}  trunk\_link               & 53.9 & 18.2 & 56.5 & 0.0 & 96.5 &  1'529  &                                                 \\
 \hspace{10pt}  primary               & 36.4 & 12.4 & 34.4 & 5.9 & 92.7 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & 33.6 & 13.9 & 31.5 & 7.3 & 94.0 &  2'430  &                                                 \\
 \hspace{10pt}  secondary               & 31.2 & 14.4 & 26.8 & 8.9 & 98.2 &  17'014  &                                                 \\
 \hspace{10pt}  secondary\_link               & 32.0 & 16.9 & 26.8 & 8.9 & 91.8 &  1'403  &                                                 \\
 \hspace{10pt}  tertiary               & 26.1 & 10.2 & 24.0 & 8.0 & 94.1 &  30'195  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 24.7 & 10.7 & 22.0 & 7.4 & 84.2 &  625  &                                                 \\
 \hspace{10pt}  unclassified               & 29.7 & 16.4 & 25.6 & 0.0 & 108.2 &  4'735  &                                                 \\
 \hspace{10pt}  residential               & 22.5 & 10.4 & 19.8 & 0.0 & 102.1 &  199'183  &                                                 \\
 speed\_kph-free\_flow\_kph                & 10.7 & 12.1 & 13.7 & -85.9 & 91.3 &  268'548 &                                                 \\
 \hspace{10pt}  motorway               & 25.8 & 15.6 & 23.3 & -14.1 & 91.3 &  338  &                                                 \\
 \hspace{10pt}  motorway\_link               & -21.9 & 17.6 & -24.5 & -60.9 & 59.3 &  698  &                                                 \\
 \hspace{10pt}  trunk               & 13.6 & 15.8 & 11.4 & -42.0 & 70.8 &  1'156  &                                                 \\
 \hspace{10pt}  trunk\_link               & -11.6 & 18.0 & -14.5 & -54.1 & 50.5 &  1'529  &                                                 \\
 \hspace{10pt}  primary               & 8.5 & 12.6 & 10.3 & -52.7 & 58.5 &  9'242  &                                                 \\
 \hspace{10pt}  primary\_link               & -1.2 & 14.1 & 0.6 & -61.6 & 49.1 &  2'430  &                                                 \\
 \hspace{10pt}  secondary               & 6.9 & 14.6 & 11.3 & -60.1 & 55.8 &  17'014  &                                                 \\
 \hspace{10pt}  secondary\_link               & -1.5 & 16.9 & 3.5 & -61.2 & 30.4 &  1'403  &                                                 \\
 \hspace{10pt}  tertiary               & 18.9 & 10.4 & 21.0 & -73.0 & 62.2 &  30'195  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 6.9 & 10.8 & 9.6 & -47.8 & 27.4 &  625  &                                                 \\
 \hspace{10pt}  unclassified               & -7.3 & 16.5 & -3.3 & -85.9 & 23.6 &  4'735  &                                                 \\
 \hspace{10pt}  residential               & 10.8 & 10.4 & 13.4 & -68.9 & 62.1 &  199'183  &                                                 \\
 movie volume 00:00--24:00               &  6.9e+07 & 1.5e+07  & 7.5e+07 & 2.9e+07 & 8.4e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  8.2e+05 & 1.6e+05  & 8.2e+05 & 5.5e+05 & 1.1e+06 &  20 &                                                \\
 movie volume 03:00--06:00               &  6.2e+05 & 1.3e+05  & 6.1e+05 & 3.6e+05 & 8.7e+05 &  20 &                                                \\
 movie volume 06:00--09:00               &  4.5e+05 & 9.7e+04  & 4.4e+05 & 2.7e+05 & 6.7e+05 &  20 &                                                \\
 movie volume 09:00--12:00               &  3.4e+05 & 7.1e+04  & 3.3e+05 & 2.3e+05 & 5.1e+05 &  20 &                                                \\
 movie volume 12:00--15:00               &  2.9e+05 & 7.6e+04  & 2.8e+05 & 1.9e+05 & 4.6e+05 &  20 &                                                \\
 movie volume 15:00--18:00               &  2.9e+05 & 7.9e+04  & 2.7e+05 & 1.7e+05 & 4.5e+05 &  20 &                                                \\
 movie volume 18:00--21:00               &  3.7e+05 & 8.6e+04  & 3.4e+05 & 2.5e+05 & 5.9e+05 &  20 &                                                \\
 movie volume 21:00--24:00               &  6.6e+05 & 1.4e+05  & 6.8e+05 & 3.3e+05 & 9.7e+05 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['melbourne'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Melbourne (2021)}
\subsubsection{Road graph map Melbourne (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_melbourne_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_melbourne_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Melbourne (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_melbourne_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_melbourne_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Melbourne (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_melbourne_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_melbourne_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Melbourne (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_melbourne_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_melbourne_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_melbourne_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_melbourne_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_melbourne_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_melbourne_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / melbourne
 num\_edges                &  &  &  &  &  &  230'654 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  354 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  891 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  5383 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  766 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  13917 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  1574 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  10342 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  394 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  30552 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  1007 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  7301 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  158173 &                                                \\
 num\_nodes                &  &  &  &  &  &  103062 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.4 & 1.0 & 1.0 & 27.0 &  891'475 &                                                 \\
 num\_intersecting\_cells                & 4.2 & 3.1 & 4.0 & 0.0 & 109.0 &  230'654 &                                                 \\
 node\_degree                & 2.8 & 0.8 & 3.0 & 1.0 & 7.0 &  103'062 &                                                 \\
 length\_meters                & 105.3 & 123.1 & 81.5 & 0.1 & 5'426.2 &  230'654 & 2.4e+07                                                \\
 \hspace{10pt}  motorway               & 1'102.6 & 774.5 & 976.5 & 24.8 & 5'426.2 &  354  & 3.9e+05                                                \\
 \hspace{10pt}  motorway\_link               & 261.5 & 319.2 & 102.2 & 2.0 & 2'331.5 &  891  & 2.3e+05                                                \\
 \hspace{10pt}  trunk               & 105.4 & 139.8 & 68.1 & 0.2 & 2'184.2 &  5'383  & 5.7e+05                                                \\
 \hspace{10pt}  trunk\_link               & 36.2 & 39.8 & 22.9 & 2.8 & 507.1 &  766  & 2.8e+04                                                \\
 \hspace{10pt}  primary               & 99.4 & 115.9 & 69.4 & 0.2 & 1'799.5 &  13'917  & 1.4e+06                                                \\
 \hspace{10pt}  primary\_link               & 30.5 & 34.3 & 17.0 & 2.0 & 681.8 &  1'574  & 4.8e+04                                                \\
 \hspace{10pt}  secondary               & 86.5 & 104.6 & 64.2 & 0.4 & 1'781.7 &  10'342  & 9.0e+05                                                \\
 \hspace{10pt}  secondary\_link               & 40.3 & 28.6 & 37.1 & 4.2 & 275.1 &  394  & 1.6e+04                                                \\
 \hspace{10pt}  tertiary               & 78.5 & 111.2 & 54.4 & 0.1 & 4'322.7 &  30'552  & 2.4e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 23.2 & 25.0 & 12.7 & 0.8 & 280.4 &  1'007  & 2.3e+04                                                \\
 \hspace{10pt}  unclassified               & 153.4 & 235.0 & 89.3 & 0.6 & 3'981.2 &  7'301  & 1.1e+06                                                \\
 \hspace{10pt}  residential               & 108.6 & 99.5 & 87.7 & 0.3 & 3'312.3 &  158'173  & 1.7e+07                                                \\
 speed\_kph                & 51.1 & 6.8 & 48.7 & 4.0 & 100.0 &  230'654 &                                                 \\
 \hspace{10pt}  motorway               & 93.6 & 9.5 & 100.0 & 50.0 & 100.0 &  354  &                                                 \\
 \hspace{10pt}  motorway\_link               & 77.2 & 11.0 & 78.9 & 40.0 & 100.0 &  891  &                                                 \\
 \hspace{10pt}  trunk               & 68.6 & 9.5 & 70.0 & 40.0 & 80.0 &  5'383  &                                                 \\
 \hspace{10pt}  trunk\_link               & 65.2 & 5.0 & 65.4 & 20.0 & 100.0 &  766  &                                                 \\
 \hspace{10pt}  primary               & 62.5 & 8.3 & 60.0 & 40.0 & 100.0 &  13'917  &                                                 \\
 \hspace{10pt}  primary\_link               & 57.1 & 3.3 & 57.0 & 40.0 & 100.0 &  1'574  &                                                 \\
 \hspace{10pt}  secondary               & 58.8 & 5.9 & 60.0 & 40.0 & 100.0 &  10'342  &                                                 \\
 \hspace{10pt}  secondary\_link               & 59.4 & 2.5 & 59.6 & 40.0 & 80.0 &  394  &                                                 \\
 \hspace{10pt}  tertiary               & 51.4 & 5.8 & 51.4 & 4.0 & 100.0 &  30'552  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 54.4 & 3.0 & 54.6 & 40.0 & 80.0 &  1'007  &                                                 \\
 \hspace{10pt}  unclassified               & 49.1 & 4.8 & 49.0 & 15.0 & 100.0 &  7'301  &                                                 \\
 \hspace{10pt}  residential               & 48.7 & 2.4 & 48.7 & 5.0 & 80.0 &  158'173  &                                                 \\
 free\_flow\_kph                & 40.6 & 18.7 & 39.5 & 0.0 & 120.0 &  187'487 &                                                 \\
 \hspace{10pt}  motorway               & 91.4 & 10.0 & 96.0 & 0.0 & 101.5 &  348  &                                                 \\
 \hspace{10pt}  motorway\_link               & 76.9 & 22.7 & 82.6 & 0.0 & 103.1 &  879  &                                                 \\
 \hspace{10pt}  trunk               & 56.4 & 13.4 & 56.9 & 8.0 & 120.0 &  5'380  &                                                 \\
 \hspace{10pt}  trunk\_link               & 47.2 & 19.8 & 49.9 & 0.0 & 99.8 &  747  &                                                 \\
 \hspace{10pt}  primary               & 51.0 & 13.1 & 52.7 & 0.0 & 120.0 &  13'913  &                                                 \\
 \hspace{10pt}  primary\_link               & 46.4 & 19.6 & 47.4 & 0.0 & 98.8 &  1'516  &                                                 \\
 \hspace{10pt}  secondary               & 49.5 & 13.3 & 51.1 & 0.0 & 120.0 &  10'301  &                                                 \\
 \hspace{10pt}  secondary\_link               & 43.1 & 15.7 & 41.2 & 0.9 & 120.0 &  387  &                                                 \\
 \hspace{10pt}  tertiary               & 42.1 & 13.0 & 41.6 & 0.0 & 120.0 &  29'619  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 39.8 & 16.4 & 38.6 & 0.0 & 120.0 &  941  &                                                 \\
 \hspace{10pt}  unclassified               & 37.9 & 18.5 & 33.9 & 0.0 & 120.0 &  6'868  &                                                 \\
 \hspace{10pt}  residential               & 37.1 & 19.4 & 35.8 & 0.0 & 120.0 &  116'588  &                                                 \\
 speed\_kph-free\_flow\_kph                & 11.0 & 17.6 & 11.2 & -100.0 & 100.0 &  187'487 &                                                 \\
 \hspace{10pt}  motorway               & 2.1 & 9.0 & 2.1 & -29.2 & 100.0 &  348  &                                                 \\
 \hspace{10pt}  motorway\_link               & 0.3 & 22.8 & -0.4 & -56.0 & 78.9 &  879  &                                                 \\
 \hspace{10pt}  trunk               & 12.3 & 12.2 & 9.2 & -60.0 & 55.5 &  5'380  &                                                 \\
 \hspace{10pt}  trunk\_link               & 18.0 & 20.0 & 15.4 & -34.6 & 65.4 &  747  &                                                 \\
 \hspace{10pt}  primary               & 11.5 & 12.5 & 8.5 & -60.0 & 66.8 &  13'913  &                                                 \\
 \hspace{10pt}  primary\_link               & 10.7 & 19.8 & 9.1 & -41.8 & 57.0 &  1'516  &                                                 \\
 \hspace{10pt}  secondary               & 9.3 & 13.1 & 7.8 & -80.0 & 60.0 &  10'301  &                                                 \\
 \hspace{10pt}  secondary\_link               & 16.4 & 16.0 & 18.7 & -60.4 & 58.7 &  387  &                                                 \\
 \hspace{10pt}  tertiary               & 9.3 & 12.7 & 9.5 & -70.0 & 92.9 &  29'619  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 14.6 & 16.4 & 15.8 & -65.4 & 64.4 &  941  &                                                 \\
 \hspace{10pt}  unclassified               & 11.2 & 18.8 & 15.1 & -71.0 & 92.0 &  6'868  &                                                 \\
 \hspace{10pt}  residential               & 11.5 & 19.5 & 12.8 & -100.0 & 70.0 &  116'588  &                                                 \\
 movie volume 00:00--24:00               &  2.5e+06 & 5.2e+05  & 2.8e+06 & 1.2e+06 & 3.0e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  2.1e+04 & 4.0e+03  & 2.1e+04 & 1.5e+04 & 2.9e+04 &  20 &                                                \\
 movie volume 03:00--06:00               &  1.8e+04 & 3.7e+03  & 1.7e+04 & 1.2e+04 & 2.7e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.7e+04 & 3.2e+03  & 1.7e+04 & 1.2e+04 & 2.6e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.6e+04 & 3.4e+03  & 1.6e+04 & 1.2e+04 & 2.7e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.7e+04 & 3.1e+03  & 1.6e+04 & 1.2e+04 & 2.5e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.9e+04 & 3.6e+03  & 1.8e+04 & 1.2e+04 & 2.7e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  2.4e+04 & 5.8e+03  & 2.4e+04 & 1.2e+04 & 3.5e+04 &  20 &                                                \\
 movie volume 21:00--24:00               &  4.3e+04 & 1.1e+04  & 4.6e+04 & 1.6e+04 & 5.5e+04 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2021', 'output_folder': 'figures/speed_stats', 'city': ['moscow'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021
\clearpage\subsection{Key Figures Moscow (2021)}
\subsubsection{Road graph map Moscow (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_moscow_2021.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_moscow_2021.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Moscow (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_moscow_2021.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_moscow_2021.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Moscow (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_moscow_2021_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_moscow_2021_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Moscow (2021)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_moscow_2021_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_moscow_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_moscow_2021_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_moscow_2021_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_moscow_2021_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_moscow_2021_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2021 / moscow
 num\_edges                &  &  &  &  &  &  47'877 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  14 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  653 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  150 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  2766 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  575 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  9406 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  1461 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  11198 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  806 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  6407 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  14441 &                                                \\
 num\_nodes                &  &  &  &  &  &  22627 &                                                 \\
 num\_edges\_per\_cell                & 1.0 & 0.2 & 1.0 & 1.0 & 8.0 &  293'771 &                                                 \\
 num\_intersecting\_cells                & 6.3 & 6.2 & 4.0 & 1.0 & 144.0 &  47'877 &                                                 \\
 node\_degree                & 2.9 & 0.8 & 3.0 & 1.0 & 7.0 &  22'627 &                                                 \\
 length\_meters                & 227.8 & 280.2 & 140.5 & 1.0 & 8'043.8 &  47'877 & 1.1e+07                                                \\
 \hspace{10pt}  motorway               & 1'970.2 & 1'889.5 & 869.5 & 151.3 & 4'808.1 &  14  & 2.8e+04                                                \\
 \hspace{10pt}  trunk               & 561.1 & 840.2 & 293.3 & 4.3 & 8'043.8 &  653  & 3.7e+05                                                \\
 \hspace{10pt}  trunk\_link               & 363.9 & 332.4 & 268.5 & 9.8 & 1'612.1 &  150  & 5.5e+04                                                \\
 \hspace{10pt}  primary               & 294.2 & 371.6 & 174.6 & 1.8 & 4'378.8 &  2'766  & 8.1e+05                                                \\
 \hspace{10pt}  primary\_link               & 238.1 & 242.6 & 164.0 & 3.8 & 1'689.3 &  575  & 1.4e+05                                                \\
 \hspace{10pt}  secondary               & 209.8 & 255.6 & 115.8 & 1.0 & 3'017.5 &  9'406  & 2.0e+06                                                \\
 \hspace{10pt}  secondary\_link               & 138.4 & 165.0 & 75.8 & 4.8 & 1'564.7 &  1'461  & 2.0e+05                                                \\
 \hspace{10pt}  tertiary               & 231.5 & 270.7 & 134.7 & 1.9 & 3'168.5 &  11'198  & 2.6e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 97.5 & 123.9 & 54.8 & 3.5 & 1'141.1 &  806  & 7.9e+04                                                \\
 \hspace{10pt}  unclassified               & 220.6 & 277.7 & 131.1 & 1.4 & 3'738.3 &  6'407  & 1.4e+06                                                \\
 \hspace{10pt}  residential               & 224.9 & 217.1 & 161.8 & 1.4 & 2'427.5 &  14'441  & 3.2e+06                                                \\
 speed\_kph                & 48.6 & 11.3 & 49.0 & 5.0 & 110.0 &  47'877 &                                                 \\
 \hspace{10pt}  motorway               & 71.1 & 16.4 & 73.2 & 40.0 & 110.0 &  14  &                                                 \\
 \hspace{10pt}  trunk               & 94.1 & 12.0 & 100.0 & 40.0 & 110.0 &  653  &                                                 \\
 \hspace{10pt}  trunk\_link               & 54.1 & 5.6 & 54.5 & 30.0 & 90.0 &  150  &                                                 \\
 \hspace{10pt}  primary               & 73.8 & 6.5 & 74.1 & 40.0 & 90.0 &  2'766  &                                                 \\
 \hspace{10pt}  primary\_link               & 45.2 & 4.7 & 45.1 & 20.0 & 60.0 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 53.5 & 5.5 & 53.5 & 20.0 & 90.0 &  9'406  &                                                 \\
 \hspace{10pt}  secondary\_link               & 50.6 & 3.8 & 50.4 & 20.0 & 90.0 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 49.6 & 5.3 & 49.0 & 5.0 & 90.0 &  11'198  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 52.6 & 3.2 & 52.4 & 30.0 & 90.0 &  806  &                                                 \\
 \hspace{10pt}  unclassified               & 36.9 & 5.3 & 36.6 & 5.0 & 90.0 &  6'407  &                                                 \\
 \hspace{10pt}  residential               & 42.5 & 4.5 & 42.6 & 5.0 & 60.0 &  14'441  &                                                 \\
 free\_flow\_kph                & 35.4 & 15.8 & 32.5 & 0.0 & 120.0 &  47'501 &                                                 \\
 \hspace{10pt}  motorway               & 93.0 & 9.7 & 92.0 & 76.2 & 105.9 &  14  &                                                 \\
 \hspace{10pt}  trunk               & 73.8 & 10.7 & 76.5 & 34.8 & 100.7 &  653  &                                                 \\
 \hspace{10pt}  trunk\_link               & 63.0 & 11.7 & 62.4 & 33.7 & 100.2 &  150  &                                                 \\
 \hspace{10pt}  primary               & 51.6 & 12.5 & 51.8 & 5.6 & 82.8 &  2'766  &                                                 \\
 \hspace{10pt}  primary\_link               & 53.4 & 13.3 & 53.9 & 8.0 & 84.2 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 41.5 & 12.5 & 40.5 & 2.2 & 120.0 &  9'406  &                                                 \\
 \hspace{10pt}  secondary\_link               & 47.1 & 15.3 & 47.4 & 4.7 & 87.8 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 35.9 & 11.9 & 34.0 & 0.0 & 120.0 &  11'198  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 44.3 & 18.0 & 42.8 & 8.9 & 101.9 &  806  &                                                 \\
 \hspace{10pt}  unclassified               & 29.4 & 14.1 & 26.4 & 0.0 & 89.9 &  6'363  &                                                 \\
 \hspace{10pt}  residential               & 25.7 & 12.3 & 23.3 & 0.0 & 120.0 &  14'109  &                                                 \\
 speed\_kph-free\_flow\_kph                & 13.3 & 14.2 & 15.6 & -77.4 & 84.4 &  47'501 &                                                 \\
 \hspace{10pt}  motorway               & -21.9 & 22.0 & -18.6 & -65.9 & 15.3 &  14  &                                                 \\
 \hspace{10pt}  trunk               & 20.3 & 12.1 & 20.9 & -45.6 & 59.9 &  653  &                                                 \\
 \hspace{10pt}  trunk\_link               & -8.9 & 12.9 & -7.7 & -45.7 & 21.8 &  150  &                                                 \\
 \hspace{10pt}  primary               & 22.2 & 12.1 & 21.0 & -21.6 & 84.4 &  2'766  &                                                 \\
 \hspace{10pt}  primary\_link               & -8.2 & 14.0 & -8.7 & -39.5 & 36.2 &  575  &                                                 \\
 \hspace{10pt}  secondary               & 12.0 & 13.2 & 13.0 & -66.5 & 69.6 &  9'406  &                                                 \\
 \hspace{10pt}  secondary\_link               & 3.5 & 15.5 & 3.3 & -51.9 & 45.7 &  1'461  &                                                 \\
 \hspace{10pt}  tertiary               & 13.7 & 12.6 & 15.4 & -71.0 & 55.2 &  11'198  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 8.4 & 18.0 & 9.6 & -49.5 & 43.5 &  806  &                                                 \\
 \hspace{10pt}  unclassified               & 7.5 & 14.5 & 10.2 & -57.6 & 72.6 &  6'363  &                                                 \\
 \hspace{10pt}  residential               & 16.8 & 13.0 & 19.5 & -77.4 & 51.1 &  14'109  &                                                 \\
 movie volume 00:00--24:00               &  8.1e+07 & 4.1e+07  & 7.4e+07 & 4.7e+07 & 2.5e+08 &  20 &                                                \\
 movie volume 00:00--03:00               &  2.2e+06 & 6.2e+05  & 2.3e+06 & 7.8e+05 & 3.2e+06 &  20 &                                                \\
 movie volume 03:00--06:00               &  1.9e+06 & 5.0e+05  & 2.0e+06 & 9.8e+05 & 2.8e+06 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.7e+06 & 4.2e+05  & 1.8e+06 & 8.3e+05 & 2.4e+06 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.5e+06 & 3.6e+05  & 1.5e+06 & 7.3e+05 & 2.1e+06 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.5e+06 & 5.8e+05  & 1.4e+06 & 6.6e+05 & 3.5e+06 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.4e+06 & 5.3e+05  & 1.4e+06 & 6.6e+05 & 3.2e+06 &  20 &                                                \\
 movie volume 18:00--21:00               &  1.4e+06 & 4.9e+05  & 1.3e+06 & 7.0e+05 & 3.1e+06 &  20 &                                                \\
 movie volume 21:00--24:00               &  1.4e+06 & 5.1e+05  & 1.4e+06 & 7.1e+05 & 3.3e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2022', 'output_folder': 'figures/speed_stats', 'city': ['london'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022
\clearpage\subsection{Key Figures London (2022)}
\subsubsection{Road graph map London (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_london_2022.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_london_2022.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  London (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_london_2022.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_london_2022.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  London (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_london_2022_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_london_2022_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  London (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_london_2022_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_london_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_london_2022_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_london_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_london_2022_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_london_2022_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022 / london
 num\_edges                &  &  &  &  &  &  271'075 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  79 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  82 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  8629 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  686 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  25189 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  411 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  11275 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  110 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  23878 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  124 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  16513 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  184099 &                                                \\
 num\_nodes                &  &  &  &  &  &  116304 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.3 & 1.0 & 1.0 & 12.0 &  912'914 &                                                 \\
 num\_intersecting\_cells                & 3.6 & 3.0 & 3.0 & 0.0 & 218.0 &  271'075 &                                                 \\
 node\_degree                & 2.5 & 0.9 & 3.0 & 1.0 & 7.0 &  116'304 &                                                 \\
 length\_meters                & 98.6 & 127.4 & 69.4 & 0.2 & 11'378.3 &  271'075 & 2.7e+07                                                \\
 \hspace{10pt}  motorway               & 2'516.4 & 2'181.2 & 1'699.3 & 209.9 & 11'378.3 &  79  & 2.0e+05                                                \\
 \hspace{10pt}  motorway\_link               & 520.9 & 373.5 & 463.0 & 16.0 & 2'450.1 &  82  & 4.3e+04                                                \\
 \hspace{10pt}  trunk               & 114.3 & 205.3 & 57.4 & 0.8 & 5'262.7 &  8'629  & 9.9e+05                                                \\
 \hspace{10pt}  trunk\_link               & 124.8 & 135.0 & 56.8 & 2.1 & 912.6 &  686  & 8.6e+04                                                \\
 \hspace{10pt}  primary               & 83.2 & 116.4 & 56.4 & 0.2 & 2'633.5 &  25'189  & 2.1e+06                                                \\
 \hspace{10pt}  primary\_link               & 40.8 & 48.2 & 28.1 & 4.1 & 494.3 &  411  & 1.7e+04                                                \\
 \hspace{10pt}  secondary               & 96.8 & 131.4 & 66.5 & 0.8 & 2'407.7 &  11'275  & 1.1e+06                                                \\
 \hspace{10pt}  secondary\_link               & 28.3 & 21.2 & 24.9 & 7.0 & 122.1 &  110  & 3.1e+03                                                \\
 \hspace{10pt}  tertiary               & 112.9 & 166.6 & 73.2 & 0.7 & 3'759.8 &  23'878  & 2.7e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 40.4 & 34.5 & 29.9 & 7.9 & 215.1 &  124  & 5.0e+03                                                \\
 \hspace{10pt}  unclassified               & 117.2 & 188.0 & 68.2 & 0.9 & 3'482.8 &  16'513  & 1.9e+06                                                \\
 \hspace{10pt}  residential               & 95.5 & 85.8 & 71.6 & 0.6 & 3'545.0 &  184'099  & 1.8e+07                                                \\
 speed\_kph                & 36.8 & 7.9 & 32.2 & 3.2 & 112.7 &  271'075 &                                                 \\
 \hspace{10pt}  motorway               & 106.2 & 15.6 & 112.7 & 48.3 & 112.7 &  79  &                                                 \\
 \hspace{10pt}  motorway\_link               & 104.4 & 16.6 & 112.7 & 48.3 & 112.7 &  82  &                                                 \\
 \hspace{10pt}  trunk               & 51.1 & 12.4 & 48.3 & 3.2 & 112.7 &  8'629  &                                                 \\
 \hspace{10pt}  trunk\_link               & 57.0 & 14.3 & 48.3 & 32.2 & 112.7 &  686  &                                                 \\
 \hspace{10pt}  primary               & 42.0 & 9.6 & 48.3 & 8.0 & 96.6 &  25'189  &                                                 \\
 \hspace{10pt}  primary\_link               & 44.2 & 8.1 & 48.3 & 20.0 & 80.5 &  411  &                                                 \\
 \hspace{10pt}  secondary               & 38.9 & 8.5 & 32.2 & 30.0 & 112.7 &  11'275  &                                                 \\
 \hspace{10pt}  secondary\_link               & 39.4 & 8.5 & 40.0 & 32.2 & 64.4 &  110  &                                                 \\
 \hspace{10pt}  tertiary               & 38.5 & 8.4 & 32.2 & 8.0 & 96.6 &  23'878  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 46.1 & 11.9 & 47.0 & 32.2 & 96.6 &  124  &                                                 \\
 \hspace{10pt}  unclassified               & 35.4 & 6.9 & 32.2 & 5.0 & 96.6 &  16'513  &                                                 \\
 \hspace{10pt}  residential               & 35.1 & 5.5 & 32.2 & 8.0 & 96.6 &  184'099  &                                                 \\
 free\_flow\_kph                & 30.0 & 11.8 & 28.7 & 0.0 & 120.0 &  263'309 &                                                 \\
 \hspace{10pt}  motorway               & 104.3 & 14.4 & 110.4 & 60.2 & 119.3 &  79  &                                                 \\
 \hspace{10pt}  motorway\_link               & 92.3 & 20.2 & 99.0 & 28.2 & 117.6 &  82  &                                                 \\
 \hspace{10pt}  trunk               & 39.5 & 12.9 & 36.2 & 5.8 & 117.5 &  8'629  &                                                 \\
 \hspace{10pt}  trunk\_link               & 53.5 & 20.7 & 57.9 & 10.4 & 119.3 &  682  &                                                 \\
 \hspace{10pt}  primary               & 35.3 & 9.6 & 32.9 & 0.0 & 108.7 &  25'189  &                                                 \\
 \hspace{10pt}  primary\_link               & 31.6 & 14.3 & 28.7 & 1.9 & 80.4 &  411  &                                                 \\
 \hspace{10pt}  secondary               & 34.9 & 9.7 & 32.9 & 0.0 & 103.2 &  11'275  &                                                 \\
 \hspace{10pt}  secondary\_link               & 27.4 & 9.4 & 26.8 & 4.7 & 65.4 &  110  &                                                 \\
 \hspace{10pt}  tertiary               & 35.0 & 10.2 & 32.9 & 0.0 & 115.3 &  23'872  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 34.7 & 14.0 & 30.2 & 12.9 & 77.6 &  124  &                                                 \\
 \hspace{10pt}  unclassified               & 28.0 & 13.0 & 26.4 & 0.0 & 118.8 &  16'213  &                                                 \\
 \hspace{10pt}  residential               & 27.8 & 11.1 & 26.8 & 0.0 & 120.0 &  176'643  &                                                 \\
 speed\_kph-free\_flow\_kph                & 6.9 & 11.5 & 6.4 & -87.8 & 87.2 &  263'309 &                                                 \\
 \hspace{10pt}  motorway               & 1.9 & 12.5 & 1.6 & -38.2 & 33.9 &  79  &                                                 \\
 \hspace{10pt}  motorway\_link               & 12.1 & 17.4 & 11.1 & -13.2 & 76.2 &  82  &                                                 \\
 \hspace{10pt}  trunk               & 11.6 & 10.6 & 11.4 & -38.8 & 72.7 &  8'629  &                                                 \\
 \hspace{10pt}  trunk\_link               & 3.5 & 18.8 & 3.6 & -35.5 & 72.5 &  682  &                                                 \\
 \hspace{10pt}  primary               & 6.7 & 10.0 & 5.5 & -56.6 & 62.7 &  25'189  &                                                 \\
 \hspace{10pt}  primary\_link               & 12.5 & 14.2 & 15.6 & -32.1 & 45.5 &  411  &                                                 \\
 \hspace{10pt}  secondary               & 4.0 & 9.5 & 3.5 & -61.7 & 59.4 &  11'275  &                                                 \\
 \hspace{10pt}  secondary\_link               & 12.1 & 10.5 & 11.0 & -17.1 & 37.4 &  110  &                                                 \\
 \hspace{10pt}  tertiary               & 3.5 & 9.6 & 3.5 & -75.4 & 75.4 &  23'872  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 11.4 & 16.8 & 12.3 & -29.3 & 69.8 &  124  &                                                 \\
 \hspace{10pt}  unclassified               & 7.3 & 12.8 & 8.2 & -83.2 & 76.8 &  16'213  &                                                 \\
 \hspace{10pt}  residential               & 7.2 & 11.7 & 7.3 & -87.8 & 87.2 &  176'643  &                                                 \\
 movie volume 00:00--24:00               &  1.1e+07 & 2.8e+06  & 1.1e+07 & 5.8e+06 & 1.5e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  1.0e+05 & 1.5e+04  & 1.0e+05 & 7.1e+04 & 1.2e+05 &  20 &                                                \\
 movie volume 03:00--06:00               &  7.8e+04 & 1.1e+04  & 7.8e+04 & 5.8e+04 & 9.9e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  6.5e+04 & 7.9e+03  & 6.7e+04 & 4.9e+04 & 8.1e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  5.7e+04 & 5.8e+03  & 5.7e+04 & 4.5e+04 & 6.8e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  5.8e+04 & 8.5e+03  & 5.9e+04 & 4.0e+04 & 7.3e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  6.6e+04 & 1.2e+04  & 7.0e+04 & 3.8e+04 & 8.1e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  8.0e+04 & 1.9e+04  & 8.9e+04 & 4.5e+04 & 1.1e+05 &  20 &                                                \\
 movie volume 21:00--24:00               &  1.3e+05 & 4.7e+04  & 1.5e+05 & 4.7e+04 & 1.9e+05 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2022', 'output_folder': 'figures/speed_stats', 'city': ['madrid'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022
\clearpage\subsection{Key Figures Madrid (2022)}
\subsubsection{Road graph map Madrid (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_madrid_2022.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_madrid_2022.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Madrid (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_madrid_2022.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_madrid_2022.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Madrid (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_madrid_2022_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_madrid_2022_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Madrid (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_madrid_2022_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_madrid_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_madrid_2022_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_madrid_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_madrid_2022_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_madrid_2022_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022 / madrid
 num\_edges                &  &  &  &  &  &  143'402 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  1277 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  2647 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  1017 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  373 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  6265 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  475 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  6855 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  276 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  16147 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  310 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  5669 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  102091 &                                                \\
 num\_nodes                &  &  &  &  &  &  71757 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.4 & 1.0 & 1.0 & 10.0 &  467'013 &                                                 \\
 num\_intersecting\_cells                & 3.5 & 3.7 & 3.0 & 0.0 & 215.0 &  143'402 &                                                 \\
 node\_degree                & 3.0 & 0.7 & 3.0 & 1.0 & 8.0 &  71'757 &                                                 \\
 length\_meters                & 110.2 & 193.2 & 66.0 & 0.2 & 10'236.5 &  143'402 & 1.6e+07                                                \\
 \hspace{10pt}  motorway               & 878.7 & 842.8 & 660.3 & 6.5 & 6'969.5 &  1'277  & 1.1e+06                                                \\
 \hspace{10pt}  motorway\_link               & 343.5 & 287.4 & 286.5 & 3.7 & 3'062.2 &  2'647  & 9.1e+05                                                \\
 \hspace{10pt}  trunk               & 254.4 & 483.3 & 60.4 & 0.2 & 4'807.2 &  1'017  & 2.6e+05                                                \\
 \hspace{10pt}  trunk\_link               & 227.4 & 235.6 & 175.3 & 5.3 & 2'997.1 &  373  & 8.5e+04                                                \\
 \hspace{10pt}  primary               & 130.1 & 335.0 & 44.6 & 0.8 & 8'314.6 &  6'265  & 8.1e+05                                                \\
 \hspace{10pt}  primary\_link               & 132.5 & 135.1 & 85.7 & 2.2 & 746.7 &  475  & 6.3e+04                                                \\
 \hspace{10pt}  secondary               & 94.2 & 247.8 & 41.0 & 0.5 & 10'236.5 &  6'855  & 6.5e+05                                                \\
 \hspace{10pt}  secondary\_link               & 73.9 & 94.8 & 38.2 & 4.3 & 763.9 &  276  & 2.0e+04                                                \\
 \hspace{10pt}  tertiary               & 88.6 & 147.2 & 45.6 & 0.3 & 3'494.5 &  16'147  & 1.4e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 77.3 & 112.8 & 35.7 & 3.9 & 829.2 &  310  & 2.4e+04                                                \\
 \hspace{10pt}  unclassified               & 169.9 & 331.4 & 76.3 & 0.9 & 5'654.6 &  5'669  & 9.6e+05                                                \\
 \hspace{10pt}  residential               & 92.7 & 92.4 & 68.0 & 0.2 & 1'966.5 &  102'091  & 9.5e+06                                                \\
 speed\_kph                & 68.6 & 1'334.2 & 76.6 & 10.0 & 505'030.0 &  143'402 &                                                 \\
 \hspace{10pt}  motorway               & 98.1 & 15.5 & 100.0 & 40.0 & 120.0 &  1'277  &                                                 \\
 \hspace{10pt}  motorway\_link               & 60.4 & 13.0 & 59.2 & 20.0 & 120.0 &  2'647  &                                                 \\
 \hspace{10pt}  trunk               & 63.8 & 19.1 & 71.2 & 20.0 & 100.0 &  1'017  &                                                 \\
 \hspace{10pt}  trunk\_link               & 52.8 & 9.2 & 52.1 & 40.0 & 90.0 &  373  &                                                 \\
 \hspace{10pt}  primary               & 87.7 & 50.7 & 50.0 & 20.0 & 151.3 &  6'265  &                                                 \\
 \hspace{10pt}  primary\_link               & 48.9 & 6.8 & 49.0 & 20.0 & 90.0 &  475  &                                                 \\
 \hspace{10pt}  secondary               & 56.5 & 120.6 & 61.3 & 20.0 & 5'030.0 &  6'855  &                                                 \\
 \hspace{10pt}  secondary\_link               & 45.1 & 4.7 & 45.3 & 30.0 & 70.0 &  276  &                                                 \\
 \hspace{10pt}  tertiary               & 44.6 & 5.8 & 44.8 & 20.0 & 90.0 &  16'147  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 41.7 & 5.7 & 41.8 & 20.0 & 70.0 &  310  &                                                 \\
 \hspace{10pt}  unclassified               & 40.6 & 4.2 & 40.5 & 10.0 & 80.0 &  5'669  &                                                 \\
 \hspace{10pt}  residential               & 73.8 & 1'580.9 & 76.6 & 20.0 & 505'030.0 &  102'091  &                                                 \\
 free\_flow\_kph                & 34.8 & 17.9 & 30.6 & 0.0 & 120.0 &  141'365 &                                                 \\
 \hspace{10pt}  motorway               & 93.3 & 15.4 & 95.2 & 12.7 & 120.0 &  1'277  &                                                 \\
 \hspace{10pt}  motorway\_link               & 86.7 & 18.0 & 90.4 & 16.0 & 120.0 &  2'645  &                                                 \\
 \hspace{10pt}  trunk               & 57.1 & 24.0 & 49.4 & 18.9 & 117.6 &  1'017  &                                                 \\
 \hspace{10pt}  trunk\_link               & 76.8 & 18.3 & 81.4 & 11.8 & 113.9 &  373  &                                                 \\
 \hspace{10pt}  primary               & 42.2 & 15.9 & 38.6 & 5.4 & 120.0 &  6'261  &                                                 \\
 \hspace{10pt}  primary\_link               & 61.4 & 24.2 & 61.6 & 3.8 & 105.9 &  474  &                                                 \\
 \hspace{10pt}  secondary               & 37.9 & 13.3 & 35.3 & 5.2 & 119.1 &  6'855  &                                                 \\
 \hspace{10pt}  secondary\_link               & 49.6 & 20.1 & 46.6 & 6.4 & 90.3 &  272  &                                                 \\
 \hspace{10pt}  tertiary               & 36.2 & 13.6 & 33.9 & 2.3 & 120.0 &  16'144  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 47.3 & 22.0 & 41.9 & 8.5 & 114.8 &  307  &                                                 \\
 \hspace{10pt}  unclassified               & 43.9 & 25.0 & 34.8 & 0.0 & 120.0 &  5'448  &                                                 \\
 \hspace{10pt}  residential               & 30.8 & 13.5 & 28.7 & 0.0 & 120.0 &  100'292  &                                                 \\
 speed\_kph-free\_flow\_kph                & 33.7 & 1'343.9 & 36.6 & -100.0 & 504'986.2 &  141'365 &                                                 \\
 \hspace{10pt}  motorway               & 4.8 & 14.1 & 4.6 & -64.0 & 87.4 &  1'277  &                                                 \\
 \hspace{10pt}  motorway\_link               & -26.3 & 19.5 & -29.3 & -75.3 & 43.2 &  2'645  &                                                 \\
 \hspace{10pt}  trunk               & 6.7 & 20.4 & 3.3 & -77.6 & 51.2 &  1'017  &                                                 \\
 \hspace{10pt}  trunk\_link               & -24.1 & 19.3 & -27.2 & -73.9 & 40.3 &  373  &                                                 \\
 \hspace{10pt}  primary               & 45.5 & 50.0 & 18.0 & -72.0 & 137.7 &  6'261  &                                                 \\
 \hspace{10pt}  primary\_link               & -12.6 & 24.7 & -12.6 & -56.9 & 48.3 &  474  &                                                 \\
 \hspace{10pt}  secondary               & 18.6 & 120.7 & 17.5 & -65.8 & 4'978.7 &  6'855  &                                                 \\
 \hspace{10pt}  secondary\_link               & -4.5 & 20.0 & -2.3 & -50.3 & 39.2 &  272  &                                                 \\
 \hspace{10pt}  tertiary               & 8.3 & 14.5 & 10.9 & -80.0 & 49.9 &  16'144  &                                                 \\
 \hspace{10pt}  tertiary\_link               & -5.6 & 22.3 & 0.6 & -73.0 & 39.7 &  307  &                                                 \\
 \hspace{10pt}  unclassified               & -3.2 & 24.7 & 5.7 & -79.5 & 49.3 &  5'448  &                                                 \\
 \hspace{10pt}  residential               & 43.0 & 1'595.0 & 44.6 & -100.0 & 504'986.2 &  100'292  &                                                 \\
 movie volume 00:00--24:00               &  3.1e+07 & 1.1e+07  & 3.1e+07 & 1.7e+07 & 6.4e+07 &  20 &                                                \\
 movie volume 00:00--03:00               &  6.9e+05 & 2.8e+05  & 6.2e+05 & 3.0e+05 & 1.3e+06 &  20 &                                                \\
 movie volume 03:00--06:00               &  5.9e+05 & 2.6e+05  & 5.4e+05 & 2.4e+05 & 1.2e+06 &  20 &                                                \\
 movie volume 06:00--09:00               &  5.1e+05 & 2.5e+05  & 4.4e+05 & 1.8e+05 & 1.0e+06 &  20 &                                                \\
 movie volume 09:00--12:00               &  4.5e+05 & 2.3e+05  & 3.7e+05 & 1.7e+05 & 9.0e+05 &  20 &                                                \\
 movie volume 12:00--15:00               &  4.0e+05 & 2.2e+05  & 3.2e+05 & 1.3e+05 & 8.3e+05 &  20 &                                                \\
 movie volume 15:00--18:00               &  3.9e+05 & 2.0e+05  & 3.1e+05 & 1.3e+05 & 7.8e+05 &  20 &                                                \\
 movie volume 18:00--21:00               &  4.0e+05 & 1.9e+05  & 3.3e+05 & 1.7e+05 & 8.1e+05 &  20 &                                                \\
 movie volume 21:00--24:00               &  4.8e+05 & 1.9e+05  & 4.2e+05 & 2.7e+05 & 1.0e+06 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}

% {'data_folder': '/iarai/public/t4c/data_pipeline//release20221026_residential_unclassified/2022', 'output_folder': 'figures/speed_stats', 'city': ['melbourne'], 'num_agg': 20, 'beyond_bounding_box': False}
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022
\clearpage\subsection{Key Figures Melbourne (2022)}
\subsubsection{Road graph map Melbourne (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/road_graph_melbourne_2022.jpg}
\caption{Road graph with OSM color scheme.}
\label{figures/speed_stats/road_graph_melbourne_2022.jpg}
\end{figure}
\clearpage\subsubsection{Temporal coverage map  Melbourne (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/density_8_18_melbourne_2022.jpg}
\caption{Segment-wise temporal coverage 8am--6pm.}
\label{figures/speed_stats/density_8_18_melbourne_2022.jpg}
\end{figure}
\clearpage\subsubsection{Coverage dayline  Melbourne (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_coverage_melbourne_2022_by_highway.pdf}
\caption{
            Mean coverage. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_coverage_melbourne_2022_by_highway.pdf}
\end{figure}
\clearpage\subsubsection{Speed dayline  Melbourne (2022)}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_median_speed_kph_melbourne_2022_by_highway.pdf}
\caption{
            Mean median 15 min speeds of all intersecting cells. All data points per hour and highway (from 20 sampled days).
            }
\label{figures/speed_stats/speed_stats_median_speed_kph_melbourne_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_mean_speed_kph_melbourne_2022_by_highway.pdf}
\caption{mean 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_mean_speed_kph_melbourne_2022_by_highway.pdf}
\end{figure}
\mbox{}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figures/speed_stats/speed_stats_std_speed_kph_melbourne_2022_by_highway.pdf}
\caption{std 15 min speeds of all intersecting cells}
\label{figures/speed_stats/speed_stats_std_speed_kph_melbourne_2022_by_highway.pdf}
\end{figure}
\begin{small}
\begin{longtable}{p{4cm}rrrrrrrr}
\toprule
Attribute      & {mean} &{std} & {median}  & {min} & {max} & {data points} & {sum}  \\
\midrule
% /iarai/public/t4c/data_pipeline/release20221026_residential_unclassified/2022 / melbourne
 num\_edges                &  &  &  &  &  &  230'654 &                                                \\
 \hspace{10pt}  motorway               &  &  &  &  &  &  354 &                                                \\
 \hspace{10pt}  motorway\_link               &  &  &  &  &  &  896 &                                                \\
 \hspace{10pt}  trunk               &  &  &  &  &  &  5382 &                                                \\
 \hspace{10pt}  trunk\_link               &  &  &  &  &  &  762 &                                                \\
 \hspace{10pt}  primary               &  &  &  &  &  &  13913 &                                                \\
 \hspace{10pt}  primary\_link               &  &  &  &  &  &  1574 &                                                \\
 \hspace{10pt}  secondary               &  &  &  &  &  &  10342 &                                                \\
 \hspace{10pt}  secondary\_link               &  &  &  &  &  &  394 &                                                \\
 \hspace{10pt}  tertiary               &  &  &  &  &  &  30557 &                                                \\
 \hspace{10pt}  tertiary\_link               &  &  &  &  &  &  1001 &                                                \\
 \hspace{10pt}  unclassified               &  &  &  &  &  &  7381 &                                                \\
 \hspace{10pt}  residential               &  &  &  &  &  &  158098 &                                                \\
 num\_nodes                &  &  &  &  &  &  103062 &                                                 \\
 num\_edges\_per\_cell                & 1.1 & 0.4 & 1.0 & 1.0 & 27.0 &  891'475 &                                                 \\
 num\_intersecting\_cells                & 4.2 & 3.1 & 4.0 & 0.0 & 109.0 &  230'654 &                                                 \\
 node\_degree                & 2.8 & 0.8 & 3.0 & 1.0 & 7.0 &  103'062 &                                                 \\
 length\_meters                & 105.3 & 123.1 & 81.5 & 0.1 & 5'426.2 &  230'654 & 2.4e+07                                                \\
 \hspace{10pt}  motorway               & 1'102.6 & 774.5 & 976.5 & 24.8 & 5'426.2 &  354  & 3.9e+05                                                \\
 \hspace{10pt}  motorway\_link               & 260.7 & 318.6 & 102.0 & 2.0 & 2'331.5 &  896  & 2.3e+05                                                \\
 \hspace{10pt}  trunk               & 105.4 & 139.8 & 68.1 & 0.2 & 2'184.2 &  5'382  & 5.7e+05                                                \\
 \hspace{10pt}  trunk\_link               & 36.0 & 39.8 & 22.8 & 2.8 & 507.1 &  762  & 2.7e+04                                                \\
 \hspace{10pt}  primary               & 99.3 & 115.6 & 69.4 & 0.2 & 1'799.5 &  13'913  & 1.4e+06                                                \\
 \hspace{10pt}  primary\_link               & 30.5 & 34.3 & 17.0 & 2.0 & 681.8 &  1'574  & 4.8e+04                                                \\
 \hspace{10pt}  secondary               & 86.5 & 104.6 & 64.2 & 0.4 & 1'781.7 &  10'342  & 9.0e+05                                                \\
 \hspace{10pt}  secondary\_link               & 40.3 & 28.6 & 37.1 & 4.2 & 275.1 &  394  & 1.6e+04                                                \\
 \hspace{10pt}  tertiary               & 78.5 & 111.2 & 54.4 & 0.1 & 4'322.7 &  30'557  & 2.4e+06                                                \\
 \hspace{10pt}  tertiary\_link               & 22.9 & 24.5 & 12.7 & 0.8 & 280.4 &  1'001  & 2.3e+04                                                \\
 \hspace{10pt}  unclassified               & 155.5 & 235.7 & 91.0 & 0.6 & 3'981.2 &  7'381  & 1.1e+06                                                \\
 \hspace{10pt}  residential               & 108.5 & 99.3 & 87.6 & 0.3 & 3'312.3 &  158'098  & 1.7e+07                                                \\
 speed\_kph                & 51.1 & 6.8 & 48.7 & 4.0 & 100.0 &  230'654 &                                                 \\
 \hspace{10pt}  motorway               & 93.6 & 9.5 & 100.0 & 50.0 & 100.0 &  354  &                                                 \\
 \hspace{10pt}  motorway\_link               & 77.2 & 11.0 & 78.9 & 40.0 & 100.0 &  896  &                                                 \\
 \hspace{10pt}  trunk               & 68.6 & 9.5 & 70.0 & 40.0 & 80.0 &  5'382  &                                                 \\
 \hspace{10pt}  trunk\_link               & 65.2 & 5.0 & 65.4 & 20.0 & 100.0 &  762  &                                                 \\
 \hspace{10pt}  primary               & 62.5 & 8.3 & 60.0 & 40.0 & 100.0 &  13'913  &                                                 \\
 \hspace{10pt}  primary\_link               & 57.1 & 3.3 & 57.0 & 40.0 & 100.0 &  1'574  &                                                 \\
 \hspace{10pt}  secondary               & 58.8 & 5.9 & 60.0 & 40.0 & 100.0 &  10'342  &                                                 \\
 \hspace{10pt}  secondary\_link               & 59.4 & 2.5 & 59.6 & 40.0 & 80.0 &  394  &                                                 \\
 \hspace{10pt}  tertiary               & 51.4 & 5.8 & 51.4 & 4.0 & 100.0 &  30'557  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 54.4 & 3.0 & 54.6 & 40.0 & 80.0 &  1'001  &                                                 \\
 \hspace{10pt}  unclassified               & 49.1 & 4.8 & 49.0 & 15.0 & 100.0 &  7'381  &                                                 \\
 \hspace{10pt}  residential               & 48.7 & 2.4 & 48.7 & 5.0 & 80.0 &  158'098  &                                                 \\
 free\_flow\_kph                & 37.7 & 18.3 & 37.2 & 0.0 & 120.0 &  190'471 &                                                 \\
 \hspace{10pt}  motorway               & 87.6 & 15.0 & 94.0 & 1.9 & 100.7 &  354  &                                                 \\
 \hspace{10pt}  motorway\_link               & 73.0 & 23.1 & 80.0 & 0.0 & 100.7 &  894  &                                                 \\
 \hspace{10pt}  trunk               & 54.9 & 13.1 & 56.0 & 8.0 & 97.9 &  5'381  &                                                 \\
 \hspace{10pt}  trunk\_link               & 44.8 & 20.3 & 46.2 & 0.0 & 99.8 &  748  &                                                 \\
 \hspace{10pt}  primary               & 49.8 & 12.9 & 51.8 & 0.9 & 100.7 &  13'906  &                                                 \\
 \hspace{10pt}  primary\_link               & 45.2 & 19.1 & 44.7 & 0.0 & 96.9 &  1'527  &                                                 \\
 \hspace{10pt}  secondary               & 47.6 & 12.6 & 49.9 & 0.0 & 100.5 &  10'326  &                                                 \\
 \hspace{10pt}  secondary\_link               & 41.7 & 14.5 & 40.9 & 0.0 & 96.9 &  385  &                                                 \\
 \hspace{10pt}  tertiary               & 39.5 & 12.2 & 39.1 & 0.0 & 120.0 &  29'809  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 37.6 & 15.4 & 36.7 & 0.0 & 96.9 &  930  &                                                 \\
 \hspace{10pt}  unclassified               & 36.0 & 18.6 & 32.2 & 0.0 & 99.8 &  7'035  &                                                 \\
 \hspace{10pt}  residential               & 33.7 & 18.6 & 32.9 & 0.0 & 120.0 &  119'176  &                                                 \\
 speed\_kph-free\_flow\_kph                & 13.9 & 17.0 & 13.8 & -71.3 & 98.1 &  190'471 &                                                 \\
 \hspace{10pt}  motorway               & 6.0 & 14.9 & 2.1 & -41.8 & 98.1 &  354  &                                                 \\
 \hspace{10pt}  motorway\_link               & 4.1 & 23.3 & 1.2 & -56.9 & 78.9 &  894  &                                                 \\
 \hspace{10pt}  trunk               & 13.7 & 12.1 & 10.4 & -22.8 & 72.0 &  5'381  &                                                 \\
 \hspace{10pt}  trunk\_link               & 20.4 & 20.5 & 18.8 & -27.3 & 65.4 &  748  &                                                 \\
 \hspace{10pt}  primary               & 12.6 & 12.3 & 9.6 & -40.9 & 65.2 &  13'906  &                                                 \\
 \hspace{10pt}  primary\_link               & 11.9 & 19.1 & 11.5 & -39.9 & 57.0 &  1'527  &                                                 \\
 \hspace{10pt}  secondary               & 11.2 & 12.4 & 9.2 & -56.7 & 60.0 &  10'326  &                                                 \\
 \hspace{10pt}  secondary\_link               & 17.8 & 14.8 & 18.7 & -37.3 & 59.6 &  385  &                                                 \\
 \hspace{10pt}  tertiary               & 11.9 & 11.7 & 11.9 & -68.6 & 92.2 &  29'809  &                                                 \\
 \hspace{10pt}  tertiary\_link               & 16.8 & 15.3 & 17.5 & -42.3 & 54.6 &  930  &                                                 \\
 \hspace{10pt}  unclassified               & 13.1 & 18.9 & 16.5 & -50.8 & 75.5 &  7'035  &                                                 \\
 \hspace{10pt}  residential               & 14.8 & 18.7 & 15.5 & -71.3 & 70.0 &  119'176  &                                                 \\
 movie volume 00:00--24:00               &  1.9e+06 & 8.4e+05  & 2.1e+06 & 6.6e+05 & 4.4e+06 &  20 &                                                \\
 movie volume 00:00--03:00               &  1.9e+04 & 4.0e+03  & 2.0e+04 & 1.1e+04 & 2.9e+04 &  20 &                                                \\
 movie volume 03:00--06:00               &  1.7e+04 & 3.5e+03  & 1.8e+04 & 9.8e+03 & 2.3e+04 &  20 &                                                \\
 movie volume 06:00--09:00               &  1.7e+04 & 3.4e+03  & 1.7e+04 & 1.0e+04 & 2.2e+04 &  20 &                                                \\
 movie volume 09:00--12:00               &  1.6e+04 & 3.3e+03  & 1.6e+04 & 9.6e+03 & 2.2e+04 &  20 &                                                \\
 movie volume 12:00--15:00               &  1.5e+04 & 3.7e+03  & 1.5e+04 & 8.9e+03 & 2.3e+04 &  20 &                                                \\
 movie volume 15:00--18:00               &  1.7e+04 & 4.6e+03  & 1.8e+04 & 9.2e+03 & 2.5e+04 &  20 &                                                \\
 movie volume 18:00--21:00               &  2.3e+04 & 7.3e+03  & 2.6e+04 & 1.1e+04 & 3.2e+04 &  20 &                                                \\
 movie volume 21:00--24:00               &  3.7e+04 & 1.7e+04  & 4.5e+04 & 1.2e+04 & 6.8e+04 &  20 &                                                \\
\bottomrule
        
        \caption{Key figures for the generated data from 20 randomly sampled days.
        \textbf{num\_edges} number of edges in the street network graph;
        \textbf{num\_nodes} number of nodes in the street network graph;
        \textbf{num\_edges\_per\_cell} number of edges a cell (row,col,heading) has in its intersecting cells;
        \textbf{num\_intersecting\_cells} number of cells (row,col,heading) in an edge's intersecting cells;
        \textbf{node\_degree} number of (unique) neighbor nodes per node;
        \textbf{length\_meters} free flow speed derived from data;
        \textbf{speed\_kph} signalled speed;
        \textbf{free\_flow\_kph} free flow speed derived from data;
        \textbf{speed\_kph-free\_flow\_kph} difference;
        \textbf{movie volume} sum of volumes over all 15min volumes of all pixels.
}
\label{tab:technical_validation:stats}
\end{longtable}
\end{small}


